Butterfly Counting in Bipartite Networks

We consider the problem of counting motifs in bipartite affiliation networks, such as author-paper, user-product, and actor-movie relations. We focus on counting the number of occurrences of a "butterfly", a complete $2 \times 2$ biclique, the simplest cohesive higher-order structure in a bipartite graph. Our main contribution is a suite of randomized algorithms that can quickly approximate the number of butterflies in a graph with a provable guarantee on accuracy. An experimental evaluation on large real-world networks shows that our algorithms return accurate estimates within a few seconds, even for networks with trillions of butterflies and hundreds of millions of edges.

==> experiments.tex <==
%\begin{table*}[t!]
%	\centering
%	\resizebox{0.95\textwidth}{!}{
%		\begin{tabular}{|c| @{\extracolsep{\fill}} |c|c|c|c|c|c|}
%			\hline
%			Bipartite graph     & $|L|$  & $|R|$ & $|E|$ & $\sum_{\ell\in{}L}{d_\ell^2}$ & $\sum_{r\in{}R}{d_r^2}$ & $\bfly$ \\ \hline
%			$\prt{10^4,10}$-biclique & \num{10000} & \num{10} & \num{100000} & \num{1000000} & \num{1000000000} & \num{2249775000} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/dbpedia-location}{DBPedia-Location}    & \num{172079} & \num{53407} & \num{293697} & \num{629983} & \num{245744643} & \num{3761594} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/edit-frwiki}{Wikipedia (fr)}    & \num{288275} & \num{3992426} & \num{22090703} & \num{2186560482259} & \num{795544489} & \num{601291038864} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/munmun_twitterex_ut}{\twt}   & \num{175214} & \num{530418} & \num{1890661} & \num{74184693} & \num{1943171143} & \num{206508691} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/amazon-ratings}{Amazon}    & \num{2146057} & \num{1230915} & \num{5743258} & \num{828704126} & \num{437163474} & \num{35849304}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/livejournal-groupmemberships}{\jrn}     & \num{3201203} & \num{7489073} & \num{112307385} & \num{9565595799} & \num{5398290985343} & \num{3297158439527}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/edit-enwiki}{\wiki}     & \num{3819691} & \num{21416395} & \num{122075170} & \num{12576726351444} & \num{23256846234} & \num{2036443879822}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/delicious-ui}{\deli}     & \num{833081} & \num{33778221} & \num{101798957} & \num{85945241607} & \num{52787267117} & \num{56892252403}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/orkut-groupmemberships}{\ork}    & \num{2783196} & \num{8730857} & \num{327037487} & \num{156580049011} & \num{4900153043329} & \num{22131701213295}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/trackers-trackers}{\web}  & \num{27665730} & \num{12756244} & \num{140613762} & \num{1733678094524} & \num{211149951033914}  & \num{20067567209850}   \\ \hline
%		\end{tabular}
%	}
%	\vspace*{0.1cm}
%	\caption{Bipartite Network Datasets. $L$ and $R$ are the partitions of the vertex set and $E$ is the set of edges.
%	\label{table:graphs}}
%\end{table*}
%--------------------






We present the results of an experimental evaluation of our algorithms for butterfly counting. We implemented the different algorithms \exact, \clr, \edgSpr, \verSam, \wdgSam, \edgSam, and \fstEdg. Based on their approach, they are classified as: (1)~{}Exact Algorithm (\exact)~{}which computes the exact number of butterflies in a bipartite graph (2)~{}Sparsification-based algorithms, \clr~{}and \edgSpr, and (3)~{}Sampling algorithms, \verSam, \wdgSam, \edgSam, and \fstEdg. For comparison, we also implemented the algorithm of Wang, Fu, and Cheng~{}\cite{Wang14}, which we call as \wangExact.
We report the following statistics: (1)~{}Relative percent error of the estimate, equal to $100 \times (|\bfly - Y|) / \bfly $ where $\bfly$ is the exact number of butterflies in $G$, and $Y$ is the estimate returned by the algorithm. (2)~{}The time taken by the algorithm. For each data point, we report the median of the fifteen trials.


%--------------



%-------------------------------------------------
\subsection{Sampling Algorithms}
%-------------------------------------------------


%--------------------
%--------------------






%To resolve this issue, we can approximate the number of butterflies containing a sampled edge. This approximation helps accelerate counting butterflies that contain an edge. By integrating this approximation procedure and the Algorithm \edgSam, more edges can be sampled which \red{results in higher accuracy}. 
%\cref{table:exact} shows the running time of two exact algorithms. For all graphs, our method, which chooses one side of a bipartite graph according to the total computation cost, works better than Wang et al's algorithm.\cite{Wang14}.
%\input{charts/BSvsIM}
%-------------------------------------------------
\subsection{Sparsification Algorithms}
%-------------------------------------------------

%\cref{fig:core1} \cref{figure:deli-sprs-err-time,figure:ork-sprs-err-time,figure:jrn-sprs-err-time,figure:web-sprs-err-time,figure:wiki-sprs-err-time} demonstrate that \edgSpr~{}yields less than one percent error after $4$ seconds. However, \clr, on some graphs such as \web~{}and \wiki, does not yield results with high accuracy in the first $30$ seconds of its execution.
%\cref{figure:deli-sprs-time-prob,figure:ork-sprs-time-prob,figure:jrn-sprs-time-prob,figure:web-sprs-time-prob,figure:wiki-sprs-time-prob} show that the runtime to sample bipartite graphs for a range of sampling probability $p$. As \clr~{}and \edgSpr~{}invoke Algorithm \exact~{}right after the sampled graph is built, the time taken for both is expected to be similar. \cref{figure:deli-sprs-time-prob,figure:jrn-sprs-time-prob,figure:ork-sprs-time-prob,figure:web-sprs-time-prob,figure:wiki-sprs-time-prob} confirm the runtime of both sparsification algorithms is in the same order. \cref{figure:deli-sprs-time-prob} shows that, for any sampling probability $p$, the runtime of algorithms in \deli~{}is higher than the runtime of \wiki~{}and \jrn, while the number of edges in \deli is fewer. The reason is because sparsification algorithms call \exact, whose time complexity is $\bigO\left( \min \left(\sum_{\ell \in L}{d_\ell^2},  \sum_{r \in R}{d_r^2}\right)\right)$. According to the \cref{table:graphs}, the runtime of \exact~{}in \deli~{}is expected to be higher than its runtime in \jrn~{}and \wiki.
%The results show that \edgSpr~{}performs much better than \clr.
%Explain the plots and summarize the results.
%\red{What are the predictions for the actual graphs used? Present the table on the different terms in the max here.
%Use it to argue why edge can be expected to perform as well as colorful.}

==> sampling.tex.bak.tex <==
%------------------------------------------------------------------------------
%\section{Approximate Butterfly Counting Using Sampling}
\section{Approximation by Sampling}
\label{sec:sampling}
%WE SURVEY POPULAR TECHNIQUES USED FOR APPROXIMATE MOTIF COUNTING IN LARGE NETWORKS FOR BIPARTITE GRAPHS. WE ANALYZE THEM AS WELL.
%------------------------------------------------------------------------------

In this section, we present approaches to approximating $\bfly(G)$ using random sampling. The intuition behind sampling is to examine a randomly sampled subgraph of $G$ and compute the number of butterflies in the subgraph to derive an estimate of $\bfly(G)$. Since the subgraph is typically much smaller than $G$, it is less expensive to perform an exact computation. The size of the chosen subgraph, the cost of computing on it, and the accuracy of the estimate vary according to the method by which we choose the random subgraph. 
% and is inexpensive for exact computation.
%Depending on how often a butterfly is observed in the sampled subgraph, we estimate the total number of butterflies in the entire graph. \textit{This sampling process can be repeated multiple times, and averaged, in order to get a better accuracy.} 
%There are three popular techniques that have been shown to be simple and effective: 
%Here we adapt those three approaches for approximate butterfly counting in a bipartite network and analyze their variances.
%We obtain an average number of butterflies per vertex upon examining multiple samples, and extrapolate this number to get an approximation.
%Literature is rich with various sampling approaches to approximately count the graph motifs such as triangles and small cliques in unipartite graphs.

We consider three natural sampling methods: vertex sampling, edge sampling, and wedge (two path) sampling.
In \verSam, the subgraph is chosen by first choosing a vertex in the graph uniformly at random, followed by the induced subgraph on the 2-neighborhood of the vertex.
In \edgSam, a random edge in the graph is chosen, followed by the induced subgraph on the union of the 1-neighborhoods of the two endpoints of the edge.
In \wdgSam, a random wedge (path of length two) is chosen, followed by the induced subgraph on the  intersection of the 1-neighborhoods of the two endpoints of the wedge.
While the methods themselves are simple, the analysis of their accuracy is challenging. We present the methods in greater detail below.
%For each algorithm, we present a detailed theoretical analysis.
%where we choose a random vertex and then count the number of butterflies that contain this vertex.
%Next, we present the \edgSam~method, where we choose a random edge and consider the butterflies that contain this edge.
%We then present the \wdgSam~ method, where we choose a random wedge (path of length two) is chosen and count the number of butterflies that contain this wedge. 

%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{figure*}[ht!]
\centering
\resizebox{0.8\linewidth}{!}{
\subfloat[][{{{\Large Type $0v$: No vertex in common}}}]{\includegraphics[width=0.33\textwidth]{figureTex/NoVertex}\label{verSamA}}~{}~{}
\hspace{3ex}
\subfloat[][{Type $1v$: One vertex in common}]{\includegraphics[width=0.33\textwidth]{figureTex/OneVer2}\label{verSamB}}~{}~{}
\hspace{3ex}
\subfloat[][{Type $2v$: Two vertices in common but no edge}]{\includegraphics[width=0.33\textwidth]{figureTex/TwoVerNoEdg}\label{verSamC}}~{}~{}
\hspace{3ex}
\subfloat[][{Type $1e$: One edge in common}]{\includegraphics[width=0.33\textwidth]{figureTex/OneEdg}\label{verSamD}}~{}~{}
\hspace{3ex}
\subfloat[][{Type $1w$: One wedge in common}]{\includegraphics[width=0.33\textwidth]{figureTex/TwoEdg}\label{verSamE}}
}
\caption{A pair of butterflies in $G$ can belong to one of the above types.}
\end{figure*}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Vertex Sampling}
%---------------------------------------
The idea in \verSam~{}is to sample a random vertex $v$ and count the number of butterflies that contain $v$ -- this is accomplished by counting the number of butterflies in the induced subgraph consisting of the 2-neighborhood of $v$ in the graph. We show that the algorithm, described in \cref{algo:versamp}, yields an unbiased estimate of $\bfly(G)$, and also analyze the variance of the estimate. The variance is reduced by taking the mean of multiple independent runs of the estimator.
%------------------------------------------------
\begin{algorithm}[t]
    \DontPrintSemicolon
    \KwIn{A bipartite graph $G = (V, E)$}
    \KwOut{An estimate of $\bfly(G)$}
    Choose a vertex $v$ from $V$ uniformly at random.\;
    $\bfly_v \gets \pervertex~(v, G)$~\tcp*{\cref{algo:local-verBFC}}
%    Compute $\bfly_v$ using \cref{algo:local-verBFC} for local (per-vertex) butterfly counting \;
    \Return $\bfly_v \cdot n/4$
    \caption{\verSam~(single iteration)
    \label{algo:versamp}}
\end{algorithm}
%------------------------------------------------
%------------------------------------------------
%------------------------------------------------
Let $Y_V$ denote the return value of \cref{algo:versamp}. Let $p_V$ denote the number of pairs of butterflies in $G$ that share a single vertex.
%------------------
\begin{lem}
%\label{lem:versamp-exp}
\label{lem:versamp}
$\expec{Y_V} = \bfly$, and $\var{Y_V} \le \frac{n}{4}(\bfly + p_V)$
\end{lem}
%------------------------------------------------
%------------------------------------------------
\begin{proof}
Consider that the butterflies in $G$ are numbered from $1$ to $\bfly$.
Let $X$ denote $\bfly_v$, the number of butterflies that contain the sampled vertex $v$.
For $i = 1, \ldots, \bfly$, let $X_i$ be an indicator random variable equal to $1$ if the $i^{\text{th}}$ butterfly includes the vertex $v$.
We have $X = \sum_{i=1}^{\bfly} X_i$. Since each butterfly has exactly four vertices in $V$, we have $\expec{X_i} = \prob{X_i=1} = 4/n$.
We further have $\expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{n}$.
Since $Y_V = X \cdot \frac{n}{4}$, it follows that $\expec{Y_V} = \bfly$.
%\end{proof}
%------------------------------------------------

In order to compute the variance of $Y_V$, we consider the joint probabilities of different butterflies being sampled together. The set of all pairs of butterflies are partitioned into different types as follows. This partitioning will help not only with analyzing this algorithm, but also in subsequent sampling algorithms. A pair of butterflies is said to be of type:
\begin{itemize}
\setlength\itemsep{0pt}
\item $0v$ if they share zero vertices (\cref{verSamA})
\item $1v$ if they share one vertex (\cref{verSamB})
\item $2v$ if they share two vertices but no edge (\cref{verSamC})
\item $1e$ if they share two vertices and exactly one edge (\cref{verSamD})
\item $1w$ if they share three vertices and two edges i.e. share a wedge (\cref{verSamE})
\end{itemize}
It can be verified that every pair of distinct butterflies must be one of the above types $\{0v,1v,2v,1e,1w\}$, and other combinations such as three vertices and more than two edges are not possible. For each type $t \in \{0v,1v,2v,1e,1w\}$, let $p_t$ denote the number of pairs of butterflies of that type. Thus $p_{0v} + p_{1v} + p_{2v} + p_{1e} + p_{1w} = {\bfly\choose{2}}$.  Let $p_V = p_{1v} + p_{2v} + p_{1e} + p_{1w}$ be the number of pairs of butterflies that share at least one vertex.
%------------------------------------------------
%\begin{lem}\label{lem:versamp-var}
%\end{lem}
%------------------------------------------------
%------------------------------------------------
%\begin{proof}
%\erdem{This can be omitted, not sure though}
%\erdem{Just keep one proof that uses Fig.3 in the paper. Put the rest in appendix or remove.}
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y_V} &= \var{\frac{n}{4}\sum_{i=1}^{\bfly}{X_i}} = \frac{n^2}{16} \var{\sum_{i=1}^{\bfly}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov(i, j)} \\
     &= \frac{n^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr}\right] \\
     %&= \frac{n^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr\expec{X_i^2} - \expec{X_i}^2\rbr} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr}\right] \\
     &= \frac{n^2}{16}\left[\bfly \lbr\frac{4}{n} - \frac{16}{n^2}\rbr + \sum_{i\neq{}j}{\lbr\expec{X_iX_j} - \expec{X_i}\expec{X_j}\rbr}\right]
  \end{aligned}
  \end{equation*}
\end{small}
%In order to compute $\sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr}$, we examine all kinds of butterfly pairs:
Consider the different types of butterfly pairs $(i,j)$:
\begin{itemize}
\setlength\itemsep{0pt}
\item
Type $0v$, there is zero probability of $i$ and $j$ being counted within $\bfly_v$, hence $\expec{X_i X_j} =  0$, $\Cov\lbr X_i, X_j \rbr = -{16}/{n^2}$
\item
Type $1v$, $\E[X_iX_j] = \Pr[X_i=1] \Pr[X_j=1 \vert X_i=1] = ({4}/{n})({1}/{4}) = {1}/{n}$. $\Cov\lbr X_i,X_j \rbr= {1}/{n} - {16}/{n^2}$.
\item
Type $2v$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{n})({1}/{2}) = {2}/{n}$.  $\Cov\lbr X_i,X_j \rbr= {2}/{n} - {16}/{n^2}$.
\item
Type $1e$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{n})({1}/{2}) = {2}/{n}$. $\Cov\lbr X_i,X_j \rbr= {2}/{n} - {16}/{n^2}$.
\item
Type $1w$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{n})({3}/{4}) = {3}/{n}$. $\Cov\lbr X_i,X_j \rbr= {3}/{n} - {16}/{n^2}$.
\end{itemize}
By adding up the different contributions, we arrive:
\begin{small}
      \begin{equation*}
      \begin{aligned}
        \Var[Y_V]  %&=  \frac{n^2}{16}\bigg[\bfly \lbr\frac{4}{n} - \frac{16}{n^2}\rbr - p_{0v}\frac{16}{n^2} + p_{1v}(\frac{1}{n}  - \frac{16}{n^2})  \\
                      %&  + p_{2v}\lbr\frac{2}{n} - \frac{16}{n^2}\rbr + p_{1e}\lbr\frac{2}{n} - \frac{16}{n^2}\rbr + p_{1w}\lbr\frac{3}{n} - \frac{16}{n^2}\rbr\bigg]\\
         %& \leq \frac{n^2}{16}\left[\frac{4}{n}\lbr\bfly + p_{1v} + p_{2v} + p_{1e} + p_{1w}\rbr - {\bfly\choose{2}}\frac{16}{n^2}\right]\\
         & \le \frac{n}{4}\lbr\bfly + p_{1v} + p_{2v} + p_{1e} + p_{1w}\rbr - {\bfly\choose{2}} \leq \frac{n}{4}\lbr\bfly + p_V\rbr
      \end{aligned}
      \end{equation*}
\end{small}
\end{proof}
%------------------------------------------------
Let $Z$ be the  average of $\alpha = \frac{8n}{\epsilon^2\bfly}\left(1 + \frac{p_V}{\bfly} \right)$ independent instances of $Y_V$. Using $\Var[Z] = \Var[Y_V] / \alpha$
and Chebyshev's inequality:
  \begin{equation*}
  \begin{aligned}
     \prob{|Z - \bfly| \geq \epsilon\bfly}  &\leq \frac{\Var[Z]}{\epsilon^2{}\bfly^2} = \frac{\Var[Y_V]}{\alpha\epsilon^2{}\bfly^2}
     \leq \frac{n(\bfly + p_V)}{4\alpha\epsilon^2{}\bfly^2} = \frac{1}{32}
  \end{aligned}
  \end{equation*}
We can turn the above estimator that yields an $\epsilon$ relative error with probability $1/32$ into an $(\epsilon,\delta)$ estimator by taking the median of $\bigO(\log(1/\delta))$ estimators, using a standard analysis based on Chernoff bounds (see~\cite{MUbook05}, Chapter 4).
%---------------
\begin{lem}
There is an algorithm that uses $\tilde{\bigO}\left(\frac{n}{\bfly}\left(1 + \frac{p_V}{\bfly} \right) \right)$
iterations~\footnote{We use the notation $\tilde{\bigO}(f)$ to suppress the factor $\frac{\log(1/\delta)}{\epsilon^2}$,
i.e. mean $\bigO\left(f \cdot \frac{\log(1/\delta)}{\epsilon^2}\right)$}
 of \textnormal{\verSam} (\cref{algo:versamp}) and yields an $(\epsilon,\delta)$-estimator of $\bfly(G)$ using expected time $\tilde{\bigO}\left(\frac{m\Delta}{\bfly}\left(1 + \frac{p_V}{\bfly} \right) \right)$. Expected additional space is $\bigO\left(\frac{m\Delta}{n}\right)$.
\end{lem}
%------------
\begin{proof}
An iteration of \textnormal{\verSam} samples a vertex $v$ and calls \textnormal{\pervertex} (\cref{algo:local-verBFC}) for local butterfly counting once, which takes $\bigO(|\Gamma^2_v|)$ time. Hence, the expected runtime of an iteration is $\bigO\left(\expec{|\Gamma^2_v|}\right)$, where the expectation is taken over a uniform random choice of a vertex. We note that $|\Gamma^2_v| \le d_v~\Delta$ where $d_v$ is $v$'s degree and $\Delta$ is the maximum degree in the graph. Thus $\expec{|\Gamma^2_v|} \le \sum_{v \in V} \frac{1}{n} d_v \Delta = \frac{\Delta}{n} \sum_{v \in V} d_v = \frac{m\Delta}{n}$.
The space of \verSam~{}is same with \textnormal{\pervertex} (\cref{algo:local-verBFC}); $\bigO(|\Gamma_v^2|)$ for handling vertex $v$. The expected value is $\bigO(\frac{m\Delta}{n})$.%Note that the space cost is in addition to the cost of storing the graph itself, which is only needed as read-only access.
\end{proof}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Edge Sampling}
In this algorithm, the idea is to sample a random edge and count the number of butterflies that contain this edge, using \peredge~(\cref{algo:local-edgBFC}).
We present \edgSam~ in~\cref{algo:edgsamp}, and state its properties.
The proofs of the lemmas are omitted due to space constraints, and can be found in the full version~\cite{fullversion}.
% of \cref{lem:edgsamp} is along similar lines to the proof of \cref{lem:versamp-exp},\cref{versamp-var}, and can be found in the full version of the paper~\cite{fullversion}

% describes the \edgSam~algorithm. We show that \edgSam~yields an unbiased estimate of $\bfly(G)$.
%-----------------------------------------------------------------------------------------
\begin{algorithm}[t!]
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \Input{A bipartite graph $G = (V, E)$}
    \KwOut{An estimate of $\bfly(G)$}
    Choose an edge $e$ from $E$ uniformly at random.\;
    $\bfly_e \gets \peredge~(e, G)$~\tcp*{\cref{algo:local-edgBFC}}\label{ln:esmp}
%    Compute $\bfly_e$ using \cref{algo:local-edgBFC}\;
    \Return $\bfly_e  \cdot m/4$
    \caption{\edgSam~(single iteration)
    \label{algo:edgsamp}}
\end{algorithm}
%-----------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------
%------------------------------------------------

Let $Y_E$ denote the return value of \textnormal{\edgSam} (\cref{algo:edgsamp}). 
Let $p_E$ be the number of pairs of butterflies that share at least one edge. Then, $p_E = p_{1e}+p_{1w}$.
\begin{lem}
\label{lem:edgsamp}
$\expec{Y_E} = \bfly$ and $\var{Y_E} \le \frac{m}{4}(\bfly + p_E)$
\end{lem}
%------------------------------------------------

%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%------------------------------------------------
\myremove{
\begin{proof}
\erdem{This can be omitted}
Consider that the butterflies in $G$ are numbered from $1$ to $\bfly$.
Let $X$ denote $\bfly_e$, when edge $e$ is chosen randomly from $E$.
For $i = 1, \ldots, \bfly$, let $X_i$ be an indicator random variable. It is $1$ if edge $e$ is contained in butterfly $i$, and $0$ otherwise.
We have $X = \sum_{i=1}^{\bfly} X_i$. Since each butterfly has exactly four edges in $E$, we have $\prob{X_i=1} = 4/m$.
\begin{align*}
\expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{m}
\end{align*}
Since $Y_E = X \cdot \frac{m}{4}$, it follows that $\expec{Y_E} = \bfly$.
\end{proof}
}
%------------------------------------------------

\myremove{
\begin{proof}
Proceeding similar to proof of \cref{lem:versamp-var}:
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y_E} &= \var{\frac{m}{4}\sum_{i=1}^{\bfly}{X_i}} = \frac{m^2}{16} \var{\sum_{i=1}^{\bfly}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov\lbr i, j\rbr } \\
     &= \frac{m^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr }\right] \\
%     &= \frac{m^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr \expec{X_i^2} - \expec{X_i}^2\rbr } + \sum_{i\neq{}j}{\Cov\lbr i, j\rbr }\right] \\
     &= \frac{m^2}{16}\left[\bfly  \lbr \frac{4}{m} - \frac{16}{m^2}\rbr  + \sum_{i\neq{}j}{\lbr \expec{X_iX_j} - \expec{X_i}\expec{X_j}\rbr }\right]
  \end{aligned}
  \end{equation*}
\end{small}
%  To compute $\sum_{i\neq{}j}{(\expec{X_iX_j} - \expec{X_i}\expec{X_j})}$ we need to consider the different types of pairs of butterflies separately.     %\item
For each type of butterfly pair, we have the following:
\begin{itemize}
\item
Type $0v$, $1v$, or $2v$: there is zero probability of $i$ and $j$ being counted within $\bfly_e$, and hence $\expec{X_i X_j} = 0$. $\Cov \lbr X_i, X_j \rbr = -{16}/{m^2}$
\item
Type $1e$: $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{m})({1}/{4}) = {1}/{m}$. $\Cov\lbr X_i,X_j \rbr= {1}/{m} - {16}/{m^2}$
\item
Type $1w$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{m})({2}/{4}) = {2}/{m}$. $\Cov\lbr X_i,X_j \rbr= {2}/{m} - {16}/{m^2}$
\end{itemize}
\begin{equation*}
  \begin{aligned}
    \Var[Y_E]  &=  \frac{m^2}{16}\bigg[\bfly \lbr \frac{4}{m} - \frac{16}{m^2}\rbr  - p_{0v}\frac{16}{m^2} - p_{1v}\frac{16}{m^2}  \\
                  &  - p_{2v}\frac{16}{m^2} + p_{1e}\lbr \frac{1}{m} - \frac{16}{m^2}\rbr  + p_{1w}\lbr \frac{2}{m} - \frac{16}{m^2}\rbr \bigg]\\
     & \leq \frac{m^2}{16}\left[\frac{4}{m}\lbr \bfly + p_{1e} + p_{1w}\rbr  - {\bfly\choose{2}}\frac{16}{m^2}\right]\\
     & = \frac{m}{4}\lbr \bfly + p_{1e} + p_{1w}\rbr  - {\bfly\choose{2}} \leq \frac{m}{4}\lbr \bfly + p_E\rbr
  \end{aligned}
\end{equation*}
\end{proof}
}

%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%By taking averages and medians as in Vertex sampling, we arrive at the following result, whose proof can be found in the full version.
\myremove{
Let $Z$ be the  average of $\alpha = ({8m}\left(1 + {p_E}/{\bfly}\right))/{(\epsilon^2\bfly)}$ independent instances of $Y_E$.
%We have $\Var[Z] = \Var[Y_E] / \alpha$.
%= \Var[\frac{1}{\alpha}\sum_{i=1}^{\alpha}Y_E] = \frac{1}{\alpha^2}\sum_{i=1}^{\alpha}{\Var[Y_E]} = \frac{\Var[Y_E]}{\alpha}$.
Using Chebyshev's inequality:
  \begin{equation*}
  \begin{aligned}
     \prob{|Z - \bfly| \geq \epsilon\bfly}  &\leq \frac{\Var[Z]}{\epsilon^2{}\bfly^2} = \frac{\Var[Y_E]}{\alpha\epsilon^2{}\bfly^2}
     \leq \frac{m(\bfly + p_E)}{4\alpha\epsilon^2{}\bfly^2} = \frac{1}{32}
  \end{aligned}
  \end{equation*}
%We can turn the above estimator that yields an $\epsilon$ relative error with probability $1/32$ into an $(\epsilon,\delta)$ estimator by taking the median of $O(\log(1/\delta))$ estimators, using standard analysis (see for e.g.~{}\cite{MUbook}, Chapter 4).
}
%---------------
\begin{lem}
Using $\tilde{\bigO}\left(\frac{m}{\bfly}\left(1 + \frac{p_E}{\bfly} \right)\right)$ iterations of \textnormal{\edgSam} yields an $(\epsilon,\delta)$-estimator of $\bfly(G)$ using time $\tilde{\bigO}\left(\frac{m^2 \Delta}{n\bfly}\left(1 + \frac{p_E}{\bfly} \right)\right)$. The additional space complexity is $\bigO\left(\frac{m\Delta}{n}\right)$.
\end{lem}
%------------

\myremove{
\begin{proof}
\erdem{This can be omitted}
Each iteration of the \edgSam~{}algorithm counts $\bfly_e$ for a randomly chosen $e$. Similar to the analysis of \verSam, the expected time of an iteration is $\bigO(m\Delta/n)$. Hence, the runtime follows. The space complexity is the space taken by \cref{algo:local-edgBFC}, which is $\bigO(m\Delta/n)$.
\end{proof}
}
%Note that the space cost in the above lemma is in addition to the cost of storing the graph itself, which is only needed as read-only access.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Wedge Sampling}

%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \Input{A bipartite graph $G = (V, E)$}
    \KwOut{An estimate of $\bfly(G)$}
    $\wdg \gets \sum_{u \in V}{{d_u\choose {2}}}$~\tcp*{number of wedges}
    Choose a vertex $u \in V$ with probability ${{d_u\choose {2}}} / \wdg$\;
    Choose two distinct vertices $v, w \in \Gamma_u$ uniformly at random\;
    $\beta \gets |\Gamma_v \cap \Gamma_w| - 1$~\tcp*{\# butterflies that has $(u, v, w)$}
    \Return $\beta \cdot \wdg/4$\;
    \caption{\wdgSam~(single iteration)}
    \label{algo:wdgsamp}
\end{algorithm}
%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

In \wdgSam, we first choose a random ``wedge", a path of length two in the graph.
This already yields three vertices that can belong to a potential butterfly.
Then we count the number of butterflies that contain this wedge by finding the intersection of the neighborhoods of the two endpoints of the wedge. %vertices that are not connected in the wedge.
\cref{algo:wdgsamp} describes the \wdgSam~{}algorithm. The correctness and complexity are stated here, with proofs deferred to the full version~\cite{fullversion}.
Let $Y_W$ denote the return value of \cref{algo:wdgsamp}. 

\myremove{
\begin{lem}
The wedge $(u, v, w)$ in lines 2 and 3 of \cref{algo:wdgsamp} is chosen uniformly at random from the set of all wedges in $G$.
\end{lem}

\begin{proof}
In order to choose the wedge $(u, v, w)$, vertex $u$ must be chosen in step (2), followed by vertices $v$ and $w$ in step (3).
The probability is $({d_y \choose 2}/\wdg) \cdot (1/{d_y \choose 2}) = 1/\wdg$, showing that a wedge is
sampled uniformly at random.
%\red{$\prt{{{d_x\choose {2}}} / \wdg}\prt{1 / {{d_x\choose {2}}}} = 1/\wdg$}. The idea comes from \cite{SePiKo14}.
\end{proof}
}
%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------------------------------------------------------

\begin{lem}
\label{lem:wdgsamp}
$\expec{Y_W} = \bfly$, and $\var{Y_W} \le \frac{\wdg}{4}(\bfly + p_{1w})$.
\end{lem}

%The proof of \cref{lem:wdgsamp} can be found in the full version of the paper~\cite{fullversion}
%------------------------------------------------
%------------------------------------------------
\myremove{
\begin{proof}
\erdem{This can be omitted}
Consider that the butterflies in $G = (V, E)$ are numbered from $1$ to $\bfly$.
Suppose that $\wdg$ is the number of wedges in $G$.
For $i = 1, \ldots, \bfly$, let $X_i$ be an indicator random variable equal to $1$ if the $i^{\text{th}}$ butterfly includes wedge $x$.
Let $X$ denote the number of butterflies that contain the sampled wedge $(u, v, w)$.
We have $X = \sum_{i=1}^{\bfly} X_i$. Since each butterfly has four wedges in $G$, we have $\prob{X_i=1} = 4/\wdg$. The rest of the proof
 is similar to that of \cref{lem:versamp-exp}, and is omitted.
%  \begin{equation*}
%  \begin{aligned}
%        \expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{\wdg}
%  \end{aligned}
%  \end{equation*}
%Since $Y = X \times \frac{\wdg}{4}$, it follows that $\expec{Y} = \bfly$.
\end{proof}
}
%Let $p_w$ denote the number of pairs of butterflies that share a wedge.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%\begin{lem}
%\label{lem:wdgsamp-var}
%\end{lem}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\myremove{
\begin{proof}
\erdem{This can be omitted}
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y} &= \var{\frac{\wdg}{4}\sum_{i=1}^{\bfly}{X_i}} = \frac{\wdg^2}{16} \var{\sum_{i=1}^{\bfly}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov\lbr i, j\rbr } \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr }\right] \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr \expec{X_i^2} - \expec{X_i}^2\rbr } + \sum_{i\neq{}j}{\Cov\lbr i, j\rbr }\right] \\
     &= \frac{\wdg^2}{16}\left[\bfly \lbr \frac{4}{\wdg} - \frac{16}{\wdg^2}\rbr  + \sum_{i\neq{}j}{\lbr \expec{X_iX_j} - \expec{X_i}\expec{X_j}\rbr }\right]
  \end{aligned}
  \end{equation*}
\end{small}
 % To compute $\sum_{i\neq{}j}{(\expec{X_iX_j} - \expec{X_i}\expec{X_j})}$: {\iffalse we need to consider the different types of pairs of butterflies separately. \fi}    %\item
 For a butterfly pair $(i,j)$, we have the following options;
\begin{itemize}
\item
Type $0v$, $1v$, $2v$, or $1e$, there is zero probability of $i$ and $j$ being counted together, and hence $\expec{X_i X_j}  = 0$. We have $\Cov \lbr X_i, X_j \rbr = -{16}/{\wdg^2}$
\item
Type $1w$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{\wdg})({1}/{4}) = {1}/{\wdg}$. Therefore, $\Cov\lbr X_i,X_j \rbr= {1}/{\wdg} - {16}/{\wdg^2}$.
\end{itemize}
\begin{equation*}
  \begin{aligned}
    \Var[Y]  &=  \frac{\wdg^2}{16}\bigg[\bfly \lbr \frac{4}{\wdg} - \frac{16}{\wdg^2}\rbr  - p_{0v}\frac{16}{\wdg^2} - p_{1v}\frac{16}{\wdg^2}  \\
                  &  - p_{2v}\frac{16}{\wdg^2} - p_{1e}\frac{16}{\wdg^2} + p_{1w}\lbr \frac{1}{\wdg} - \frac{16}{\wdg^2}\rbr \bigg]\\
     & \leq \frac{\wdg^2}{16}\left[\frac{4}{\wdg}\lbr \bfly + p_{1w}\rbr  - {\bfly\choose{2}}\frac{16}{\wdg^2}\right]\\
     & = \frac{\wdg}{4}\lbr \bfly + p_{1w}\rbr  - {\bfly\choose{2}} \leq \frac{\wdg}{4}\lbr \bfly + p_{1w}\rbr
  \end{aligned}
\end{equation*}
\end{proof}
}

%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\myremove{
Let $Z$ be the  average of $\alpha = ({8\wdg}\left(1 + {p_{1w}}/{\bfly}\right))/{(\epsilon^2\bfly)}$ independent instances of $Y$.
Using Chebyshev's inequality, we arrive that $Z$ is an $(\epsilon, 1/32)$-estimator of $\bfly(G)$.
}
%We have $\Var[Z] = \Var[Y] / \alpha$.
%= \Var[\frac{1}{\alpha}\sum_{i=1}^{\alpha}Y] = \frac{1}{\alpha^2}\sum_{i=1}^{\alpha}{\Var[Y]} = \frac{\Var[Y]}{\alpha}$.
%Using Chebyshev's inequality, we have:
%  \begin{equation*}
%  \begin{aligned}
%     \prob{|Z - \bfly| \geq \epsilon\bfly}  &\leq \frac{\Var[Z]}{\epsilon^2{}\bfly^2} = \frac{\Var[Y]}{\alpha\epsilon^2{}\bfly^2}
%    \leq \frac{\wdg(\bfly + p_{1w})}{4\alpha\epsilon^2{}\bfly^2} = \frac{1}{32}
%  \end{aligned}
%  \end{equation*}

%We can turn the above estimator that yields an $\epsilon$ relative error with probability $1/32$ into an $(\epsilon,\delta)$ estimator by taking the median of $O(\log(1/\delta))$ estimators, using standard analysis (see for e.g.~{}\cite{MUbook}, Chapter 4).
%---------------
\begin{lem}
There is an algorithm that uses $\allowbreak\tilde{\bigO}\bigl(\frac{\wdg}{\bfly}\bigl(1 + \frac{p_{1w}}{\bfly} \bigr)\bigr)$
iterations of \cref{algo:wdgsamp} and yields an $(\epsilon,\delta)$-estimator of $\bfly(G)$ using time $\tilde{\bigO}\left(\frac{(\Delta + \log n)\wdg}{\bfly}\left(1 + \frac{p_{1w}}{\bfly} \right)\right)$ and space $\bigO(n)$.
\end{lem}
%------------

\myremove{
\begin{proof}
\erdem{This can be omitted}
We first consider the runtime of \cref{algo:wdgsamp}. At first glance, it looks like Steps (1) and (2) take $\bigO(n)$ time.
This can be reduced to $\bigO(\log n)$ using a pre-computation step of time $\bigO(n)$, which precomputes the value of $h$, and also stores the values of ${d_v \choose 2}$ for different vertices $v$ in an array $A[1\ldots n]$ of length $n$. We consider another array $B[1\ldots n]$, where each element $B[j] = \sum_{i=1}^j A[i]$.  When \wdgSam~{}is called, a random number $r$ in the range $\{1,2,\ldots,h\}$ is first generated, and Step (2) is accomplished through finding the smallest $j$ such that $B[j] \ge r$. Since array $B$ is sorted in increasing order, this can be done in time $\bigO(\log n)$ using a binary search. Steps (3) and (4) of \cref{algo:wdgsamp} can be performed in $\bigO(\Delta)$ time -- Step (4), for example, through storing all elements of $\Gamma_u$ in a hash set, and repeatedly querying for elements of $\Gamma_v$ in this hash set, for a total of $\bigO(d_v) = \bigO(\Delta)$ time. The additional space required by this algorithm, in addition to the stored graph itself, is $\bigO(n)$, for random sampling.
\end{proof}
}
%Note that the space cost in the above lemma is in addition to the cost of storing the graph itself, which is only needed as read-only access.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%\subsection{Comparison}
%We next compare the different sampling algorithms

\subsection{Comparison of Sampling Algorithms on Real-World Networks}
In order to understand the relation between the three sampling algorithms, we compare the variance of the estimates retuned by these algorithms. Note that each of them returns an unbiased estimate of the number of butterflies. The variance of \verSam, \edgSam, and \wdgSam~{}for different graphs are estimated and summarized in \cref{table:variance-sam}. The results show that the variances of \verSam~{}and \wdgSam~{}are much higher than the variance of \edgSam. 

%
%%-------------- old table
%\begin{table}[b!]
%	\vspace{1ex}
%	\centering
%	\resizebox{0.5\textwidth}{!}{
%		\begin{tabular}{|c| @{\extracolsep{\fill}} |c|c|c|}
%			\hline
%	\multirowcell{2.3}[1.9ex]{\diagbox[height=1.95\line]{\rlap{\enspace\raisebox{0.6ex}{Graph}}}{\raisebox{-0.5ex}{Algorithm}}} & \makecell{\verSam{}\\$(\bfly + p_v)n/4$} & \makecell{\edgSam\\$(\bfly + p_e)m/4$} & \makecell{\wdgSam\\$(\bfly + p_w)h/4$} \\\hline
%	
%			\deli & $7.928 \times 10^{26}$ & $1.628 \times 10^{18}$ & $6.033 \times 10^{23}$ \\ \hline		
%			\jrn & $5.458 \times 10^{30}$ & $5.584 \times 10^{24}$ & $2.046 \times 10^{28}$\\ \hline
%			\ork & $2.450 \times 10^{31}$ & $5.290 \times 10^{21}$ & $1.031 \times 10^{29}$ \\ \hline
%			\web & $4.742 \times 10^{33}$ & $1.073 \times 10^{22}$ & $1.940 \times 10^{33}$ \\ \hline
%			\wiki & $1.931 \times 10^{32}$ & $6.818 \times 10^{19}$ & $2.052 \times 10^{30}$\\ \hline
%	\end{tabular}}
%	\vspace{1ex}
%	\caption{Variance values for the sampling estimators given in \cref{sec:sampling} on the large graphs}\label{table:variance-sam}
%\end{table}
%%--------------



\begin{table}[t!]
\footnotesize
%\hspace{-7ex}
\centering
\begin{tabular}{|c|c|r|c|r|c|r|c|}\hline
& \multicolumn{2}{c|}{\verSam} & \multicolumn{2}{c|}{\edgSam} & \multicolumn{2}{c|}{\wdgSam} \\
& $\frac{(\bfly+p_V)n}{4}$ & error \% & $\frac{(\bfly+p_E)m}{4}$ & error \% & $\frac{(\bfly+p_{1w})h}{4}$ & error \% \\ \hline
\deli	&	$	7.9\times 10^{26}	$	&	$	495	$	&	$	1.6\times 10^{18}	$	&	$	0.022	$	&	$	6.0\times 10^{23}	$	&	$	14	$	\\ \hline
\jrn	&	$	5.5\times 10^{30}	$	&	$	709	$	&	$	5.6\times 10^{24}	$	&	$	0.717	$	&	$	2.0\times 10^{28}	$	&	$	43	$	\\ \hline
\ork	&	$	2.5\times 10^{31}	$	&	$	224	$	&	$	5.3\times 10^{21}	$	&	$	0.003	$	&	$	1.0\times 10^{29}	$	&	$	15	$	\\ \hline
\web	&	$	4.7\times 10^{33}	$	&	$	3432	$	&	$	1.1\times 10^{22}	$	&	$	0.005	$	&	$	1.9\times 10^{33}	$	&	$	2195	$	\\ \hline
\wiki	&	$	1.9\times 10^{32}	$	&	$	6824	$	&	$	6.8\times 10^{19}	$	&	$	0.004	$	&	$	2.1\times 10^{30}	$	&	$	703	$	\\ \hline
	\end{tabular}
	\vspace{1ex}
	\caption{Variance values for the sampling estimators given in \cref{sec:sampling} on the large graphs. \erdem{Errors are sqrt of variance numbers over the num of butterflies. For vertex and wedge those upper bound are correct. but i didn't understand it for edge sampling? We do have errors more than those numbers (in figs 5-8). any idea?}}\label{table:variance-sam}
\end{table}


%Let us compare the variances of \verSam~{}and \edgSam.  
The variance of \verSam~{}is proportional to $n p_V$ where $p_V$ is the number of {\em pairs of butterflies that share a vertex} and $n$ is the number of vertices. 
For the \edgSam, the variance is correlated with $m p_E$ where $p_E$ is the number of {\em pairs of butterflies that share an edge} and $m$ is the number of edges
Note that typically $\bfly \ll p_V, p_E$ and hence $\bfly + p_V \approx p_V$ and $\bfly + p_E \approx p_E$.
If two butterflies share an edge, they certainly share a vertex, hence $p_E \le p_V$. Since it is possible that two butterflies share a vertex but do not share an edge, $p_E$ could be much smaller than $p_V$. It turns out that in most of these graphs, $p_E$ was much smaller than $p_V$.
On the other hand, the number of vertices in a graph ($n$) is comparable to the number of edges ($m$). Typically $m < 10n$, and only in one case (\ork), we have $m \approx 30n$.
Thus, $n p_V \ll m p_E$ for the graphs we consider. 
As a result, the variance of \verSam~{}estimator is much larger than the variance of \edgSam{}, which is reflected clearly in \cref{table:variance-sam}. 
%This explains why \verSam~{}performs poorly when compared with \edgSam. 

Regarding the comparison of \edgSam~{}with \wdgSam, we note that the variance of \wdgSam~{}is proportional to $\wdg p_{1w}$, where $\wdg$ is the number of wedges in the graph, which is $\bigO(\sum_v d_v^2)$ and $p_{1w}$ is the number of pairs of butterflies that share a wedge.
The variance for \edgSam is correlated with $m p_E$, as mentioned above. 
$p_1w \le p_E$ since each pair of butterflies that shares a wedge also shares an edge.
At the same time, we see that $\wdg$ is substantially greater than $m$. 
Overall, the variance of \wdgSam~{}is larger than that of \edgSam, and \edgSam~{}has the smallest variance among all.
%Due to high variance on large graphs, \verSam and \wdgSam~{}do not converge to less than one percent error. In the graph \deli, the variance of \wdgSam~{}is not too much. \cref{figure:deli-sam-err-time} shows that this algorithm estimates the number of butterflies within one percent error after a few seconds.

\subsection{Runtime discussion}\label{sec:quickBFC}

Here we study the time taken by the different sampling algorithms. \cref{figure:timePerSample} presents the results for the largest five networks in our dataset.
Note that, sampling the same number vertices/edge/wedges shows that \edgSam~gives much less variance than the others.
However, \edgSam~{}requires the largest amount of time per sampling step with a significant difference. This decreases the overall efficiency of the \edgSam~{}algorithm despite its small variance observed in~\cref{table:variance-sam}. 

\begin{figure}[!t]
\centering
\resizebox{0.7\linewidth}{!}{\input{newResults/histogram/time-per-sample}}
\caption{{\small Avg. time to get one sample for sampling algorithms.}\erdem{make it smaller and also remove the fast edge sampling bars (will be shown in~\cref{sec:quickBFC})}}
\label{figure:timePerSample}
\vspace{-1ex}
\end{figure}


\subsubsection{\textnormal{\fstEdg}: Speeding up Edge Sampling}
In order to reduce the time taken by each iteration of~\edgSam, we propose another level of sampling,~\fstEdg, that estimates the number of butterflies for a given edge.
Instead of computing the exact number of butterflies for each edge $(u, v)$ (line~\ref{ln:esmp} of \edgSam~(\cref{algo:edgsamp})), we randomly choose one neighbor of $u$ and of $v$, and check if those four vertices form a butterfly.
\cref{algo:qBFC} presents the~\fstEdg algorithm.
We use it instead of the \peredge algorithm in \edgSam.
We expect that while the estimate from each iteration is less accurate than in \edgSam, each iteration is faster, so that more iterations are possible within the same time.
Overall, in large graphs, this leads to an improvement in accuracy over \edgSam. For a given edge $e$, \cref{algo:qBFC} yields an unbiased estimate of $\bfly_e$.

\begin{algorithm}[t!]
    \DontPrintSemicolon
    \KwIn{An edge $e = (v, u) \in E$ in $G = (V, E)$}
    \KwOut{An estimate of $\bfly_e$}
    Choose a vertex $w$ ($\ne v$) from $\Gamma_u$ uniformly at random\;
    Choose a vertex $x$ ($\ne u$) from $\Gamma_v$ uniformly at random\;
    \IfThen{$(u, v, w, x)$ forms a butterfly}{${\beta} \gets 1$}\;
    \lElse {${\beta} \gets 0$}
    \Return ${\beta}\cdot (d_u-1) \cdot (d_v-1)$\;
    \caption{\fstEdg~(replaces \peredge~in \edgSam)
    \label{algo:qBFC}}
\end{algorithm}

Let $Y_{FE}$ denote the return value of \cref{algo:qBFC}. 
\begin{lem}
\label{lem:fastedge-samp}
$\expec{Y_{FE}} = \bfly_e$ and $\var{Y_{FE}} \leq \bfly_e(d_u \cdot d_v)$.
\end{lem}
%------------------------------------------------
%------------------------------------------------
\begin{proof}
Consider that the butterflies include the edge $e = (u, v)$ are numbered from $1$ to $\bfly_e$.
For $i = 1, \ldots, \bfly_e$, let $X_i$ be an indicator random variable. $X_i$ is equal $1$ if the $i^{\text{th}}$ butterfly contains both sampled neighbors $w$ and $x$, otherwise $0$.
Let $X = \sum_{i=1}^{\bfly_e} X_i$. Since vertex $w$ and $x$ are chosen with probability $1/d_u$ and $1/d_v$, respectively, $\prob{X_i=1} = 1/(d_u \cdot d_v)$. Then,
\begin{align*}
  \expec{X} = \sum_{i=1}^{\bfly_e} \expec{X_i} = \sum_{i=1}^{\bfly_e} \prob{X_i=1} = \frac{\bfly_e}{d_u\cdot{}d_v}
\end{align*}
$Y_{FE} = X \cdot d_u \cdot d_v$ follows that $\expec{Y_{FE}} = \bfly_e$.
%  \begin{equation*}
%  \begin{aligned}
%        \expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{\wdg}
%  \end{aligned}
%  \end{equation*}
%Since $Y_{FE} = X \times \frac{\wdg}{4}$, it follows that $\expec{Y_{FE}} = \bfly$.
%\end{proof}
%Let $p_w$ denote the number of pairs of butterflies that share a wedge.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
For the variance,
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y_{FE}} &= \var{(d_u \cdot d_v)\sum_{i=1}^{\bfly_e}{X_i}} = (d_u \cdot d_v)^2~{}\var{\sum_{i=1}^{\bfly_e}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov\lbr i, j\rbr } \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr }\right] \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr \expec{X_i^2} - \expec{X_i}^2\rbr } + \sum_{i\neq{}j}{\Cov\lbr i, j\rbr }\right] \\
%     &= (d_v \cdot d_u)^2\left[\sum_{i=1}^{\bfly_e}{\left[\expec{X_i^2} - \expec{X_i}^2\right]} + \sum_{i \neq j}{\Cov(X_i, X_j)}\right]\\
     &= (d_u \cdot d_v)^2\left[\sum_{i=1}^{\bfly_e}{\left[\frac{1}{d_u \cdot d_v} - \frac{1}{(d_u \cdot d_v)^2}\right]} - {\bfly_e \choose {2}}\right]\\
     &\le \bfly_e \cdot d_u \cdot d_v
  \end{aligned}
  \end{equation*}
\end{small}
 % To compute $\sum_{i\neq{}j}{(\expec{X_iX_j} - \expec{X_i}\expec{X_j})}$: {\iffalse we need to consider the different types of pairs of butterflies separately. \fi}    %\item
\end{proof}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
Let $Z$ be the  average of $\alpha = 32({d_u\cdot{}d_v})/{(\epsilon^2\bfly_e)}$ independent instances of $Y_{FE}$.
Using Chebyshev's inequality, we arrive that $Z$ is an $(\epsilon, 1/32)$-estimator of $\bfly_e$.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\subsubsection{\textnormal{\fstEdg}~runtime}



\begin{table}[t!]
\footnotesize
%\hspace{-7ex}
\centering
\begin{tabular}{|c|r|r|r|}\hline
%& \multicolumn{2}{c|}{\verSam} & \multicolumn{2}{c|}{\edgSam} & \multicolumn{2}{c|}{\wdgSam} \\
%& $\frac{(\bfly+p_V)n}{4}$ & error \% & $\frac{(\bfly+p_E)m}{4}$ & error \% & $\frac{(\bfly+p_{1w})h}{4}$ & error \% \\ \hline
in & \multicolumn{2}{c|}{\edgSam} &   \\
milliseconds & with \peredge & with \fstEdg  & Speedup \\ \hline
\deli	&	$	2.61	$	&	$	0.17	$	&	$	15.4	$	\\ \hline
\jrn	&	$	172.42	$	&	$	0.48	$	&	$	357.4	$	\\ \hline
\ork	&	$	36.76	$	&	$	0.37	$	&	$	98.1	$	\\ \hline
\web	&	$	34.49	$	&	$	0.42	$	&	$	81.5	$	\\ \hline
\wiki	&	$	55.65	$	&	$	0.48	$	&	$	115.5	$	\\ \hline
\end{tabular}
\vspace{1ex}
\caption{Runtimes of \edgSam~algorithms per iteration when \peredge~and \fstEdg~are used. Speedup of the second over first is given in the last column}\label{tab:quickBFC}
\end{table}

\cref{tab:quickBFC} gives the comparison of \peredge~and \fstEdg~when they are used in the \edgSam.
We observe speedups from $15.4$ up to $357.4$ per each iteration.

\subsection{Comparing the Different Sampling-based Approaches}
We compare all the sampling algorithms: \verSam~(\cref{algo:versamp}), \edgSam~(\cref{algo:edgsamp}) with \peredge, \edgSam with~\fstEdg~(\cref{algo:qBFC}), and \wdgSam~(\cref{algo:wdgsamp}) in terms of their accuracy and efficiency. We show the results for the five large bipartite graphs. A sampling algorithm immediately starts producing estimates that typically get better as more iterations of sampling take place. We record the number of iterations and relative percent error of sampling algorithms up to 60 seconds. \cref{figure:deli-sam-err-time,figure:jrn-sam-err-time,figure:ork-sam-err-time,figure:web-sam-err-time,figure:wiki-sam-err-time} show the relative percent error with respect to the runtime.



%\begin{figure}[!t]
%\centering
%\captionsetup[subfigure]{captionskip=-3ex}
%\subfloat[\footnotesize \deli]{\input[width=0.19\linewidth]{newResults/delicious/sam-err-time}}
%\subfloat[\footnotesize \ork]{\input[width=0.19\linewidth]{newResults/orkut/sam-err-time}}
%\subfloat[\footnotesize \jrn]{\input[width=0.19\linewidth]{newResults/Journal/sam-err-time}}
%\subfloat[\footnotesize \web]{\input[width=0.19\linewidth]{newResults/trackers/sam-err-time}}
%\subfloat[\footnotesize \wiki]{\input[width=0.19\linewidth]{newResults/Wikipedia/sam-err-time}}
%\hspace{-5ex}
%\subfloat[\footnotesize \textbf{\textsc{$(2,3)$ nucleus}}]{\includegraphics[width=0.6\linewidth]{./figures/mov_23_new.pdf}}
%\hspace{-13ex}
%
%\hspace{-1ex}
%\vspace{-7.5ex}
%\caption{\footnotesize \bf Dense subgraphs for the \imdb~network. Each dot is a bipartite subgraph and edge density is color coded. $U'$ and $V'$ are the primary and secondary vertex sets and their sizes are given on the x- and y-axes. Wing decomposition results in 36 bipartite subgraphs with $\ge 0.9$ edge density that have at least 10 vertices in each side, and perform competitive to the butterfly densest subgraph~\protect{\cite{Babis15KDD}}. Other algorithms working on projections, on the right, cannot report any bipartite subgraphs in that quality.}
%\vspace{0ex}
%\label{fig:introfig}
%\end{figure}



\begin{figure*}[!t]
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/delicious/sam-err-time}}
		\caption {\deli}\label{figure:deli-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/Journal/sam-err-time}}
		\caption {\jrn}\label{figure:jrn-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/orkut/sam-err-time}}
		\caption {\ork}\label{figure:ork-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/trackers/sam-err-time}}
		\caption {\web}\label{figure:web-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/Wikipedia/sam-err-time}}
		\caption {\wiki.}\label{figure:wiki-sam-err-time}
	\end{minipage}
	\vspace{1ex}
	\caption*{{\bf Accuracy by time results for sampling algorithms.}~\fstEdg~{\bf results in less than one percent relative error within 7 seconds for all the networks.}\erdem{replace those with the new 30 trial results and edit the text as needed. And please put pdfs of the figures. we can remove one of five for brevity. Also, put those in a proper subfigure format}}
	\vspace{-1ex}
\end{figure*}

The experiments on sampling show that \verSam~{}performs poorly when compared with \edgSam~{}and \wdgSam under the same time budget. The performance of \edgSam~{}is typically (but not always) better than that of \wdgSam.
As we show in~\cref{table:variance-sam}, \edgSam~gives way better variance results than \wdgSam. However, since \wdgSam~is faster than~\edgSam per iteration, more iterations of \wdgSam~are possible given the same time budget.
For instance, applying 1000 iterations in \wiki~network results in $51\%$ error with \wdgSam~whereas the \edgSam~can yield $29\%$ error. But, the former takes $0.13$ seconds while the latter needs $33.76$ secs.
Considering all the graphs, using \fstEdg~yields the best results; \textbf{less than one percent relative error can be reported within $7$ seconds}.
%\erdem{any explanation for that? Deli, orkut, and wiki are like that. Oh ok. This is because we show the time in x-axis. We KNOW that if the same number of samples are used, edge sampling definitely outperforms wedge sampling -- I also checked the raw data. But we need to state this explicitly.}









==> sampling__vahid_sanei_s_conflicted_copy_2018-02-07_.tex <==
%------------------------------------------------------------------------------
%\section{Approximate Butterfly Counting Using Sampling}
\section{Approximation by Sampling}
\label{sec:sampling}

%WE SURVEY POPULAR TECHNIQUES USED FOR APPROXIMATE MOTIF COUNTING IN LARGE NETWORKS FOR BIPARTITE GRAPHS. WE ANALYZE THEM AS WELL.
%------------------------------------------------------------------------------

In this section, we present different approaches for approximating the $\bfly(G)$ using random sampling and investigate on real-world data.
The intuition behind sampling is to examine a randomly sampled subgraph of $G$, which can be chosen in different ways.
The subgraph is typically much smaller than $G$ and is inexpensive for exact computation.
Depending on how often a butterfly is observed in the sampled subgraph, we estimate the total number of butterflies in the entire graph.
\textit{We consider multiple samples and take their average in order to get a better accuracy.} 

Literature is rich with various sampling approaches to approximately count the graph motifs such as triangles and small cliques in unipartite graphs.
As stated in~\cref{sec:related}, there are three popular techniques that have been shown to be simple and effective: vertex sampling, edge sampling, and wedge (two path) sampling.
Here we adapt those three approaches for approximate butterfly counting in a bipartite network and analyze their variances.
We first present the \verSam~method, where we choose a random vertex and count the butterflies it participates. We obtain an average number of butterflies per vertex upon examining multiple samples, and extrapolate this number to get an approximation.
Next, we discuss the \edgSam~method. We choose a random edge and consider the butterflies that contain this edge for extrapolation.
We also introduce \wdgSam, where a random wedge (path of length two) is chosen and the number of butterflies it is contained is counted.
For each algorithm, we present a detailed theoretical analysis of the properties of the estimator.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{figure}[ht!]
\centering
\resizebox{0.99\linewidth}{!}{
\subfloat[][{\scriptsize Type $0v$: No vertex in common}]{\includegraphics[width=0.15\textwidth]{figureTex/NoVertex}\label{verSamA}}~{}~{}
\hspace{3ex}
\subfloat[][{\scriptsize Type $1v$: One vertex in common}]{\includegraphics[width=0.15\textwidth]{figureTex/OneVer}\label{verSamB}}~{}~{}
\hspace{3ex}
\subfloat[][{\scriptsize Type $2v$: Two vertices in common but no edge}]{\includegraphics[width=0.15\textwidth]{figureTex/TwoVerNoEdg}\label{verSamC}}~{}~{}
\hspace{3ex}
\subfloat[][{\scriptsize Type $1e$: One edge in common}]{\includegraphics[width=0.15\textwidth]{figureTex/OneEdg}\label{verSamD}}~{}~{}
\hspace{3ex}
\subfloat[][{\scriptsize Type $1w$: One wedge in common}]{\includegraphics[width=0.15\textwidth]{figureTex/TwoEdg}\label{verSamE}}
}
\caption{A pair of butterflies in $G$ can belong to one of the above types.\erdem{draw bigger. Throughout the paper, I used u and x to refer vertices in L, and v and w for the vertices in R. It'd be better to show them here.}
}
\end{figure}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Vertex Sampling}
The idea in \verSam~{}is to sample a random vertex $v$, and then count the number of butterflies in the induced subgraph consisting of the two-neighborhood of $v$ in the graph. Note that this is equivalent to counting the number of butterflies that contain the sampled vertex.
\cref{algo:versamp} describes the \verSam~{}algorithm. We show that this algorithm yields an unbiased estimate of $\bfly(G)$. In order to decrease the variance, we take the mean of multiple independent copies of this estimator.
%------------------------------------------------
\begin{algorithm}[t]
    \DontPrintSemicolon
    \KwIn{A bipartite graph $G = (V, E)$}
    \KwOut{An estimate of $\bfly(G)$}
    Choose a vertex $v$ from $V$ uniformly at random.\;
    $\bfly_v \gets \pervertex~(v, G)$~\tcp*{\cref{algo:local-verBFC}}
%    Compute $\bfly_v$ using \cref{algo:local-verBFC} for local (per-vertex) butterfly counting \;
    \Return $\bfly_v \cdot n/4$
    \caption{\verSam~(single iteration)
    \label{algo:versamp}}
\end{algorithm}
%------------------------------------------------
%------------------------------------------------
%------------------------------------------------
\begin{lem}
\label{lem:versamp-exp}
Let $Y$ denote the return value of \cref{algo:versamp}. Then, $\expec{Y} = \bfly$.
\end{lem}
%------------------------------------------------
%------------------------------------------------
\begin{proof}
Consider that the butterflies in $G$ are numbered from $1$ to $\bfly$.
Let $X$ denote $\bfly_v$, the number of butterflies that contain the sampled vertex $v$.
For $i = 1, \ldots, \bfly$, let $X_i$ be an indicator random variable equal to $1$ if the $i^{\text{th}}$ butterfly includes the vertex $v$.
We have $X = \sum_{i=1}^{\bfly} X_i$. Since each butterfly has exactly four vertices in $V$, we have $\expec{X_i} = \prob{X_i=1} = 4/n$.\\
$\expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{n}$.
Since $Y = X \cdot \frac{n}{4}$, it follows that $\expec{Y} = \bfly$.
\end{proof}
%------------------------------------------------
\noindent In order to compute the variance of $Y$, we need to consider the joint probabilities of different butterflies being sampled together. To help with this, we partition the set of all pairs of butterflies into different types as follows.  This partitioning will help not only with this algorithm, but also in subsequent sampling algorithms. A pair of butterflies is said to be of type:
\begin{itemize}
\setlength\itemsep{0pt}
\item $0v$ if they share zero vertices (\cref{verSamA})
\item $1v$ if they share one vertex (\cref{verSamB})
\item $2v$ if they share two vertices but no edge (\cref{verSamC})
\item $1e$ if they share two vertices and exactly one edge (\cref{verSamD})
\item $1w$ if they share three vertices and two edges i.e. share a wedge (\cref{verSamE})
\end{itemize}
It can be verified that every pair of distinct butterflies must be one of the above types $\{0v,1v,2v,1e,1w\}$, and other combinations such as three vertices and more than two edges are not possible. For each type $t \in \{0v,1v,2v,1e,1w\}$, let $p_t$ denote the number of pairs of butterflies of that type. Thus $p_{0v} + p_{1v} + p_{2v} + p_{1e} + p_{1w} = {\bfly\choose{2}}$.  Let $p_V = p_{1v} + p_{2v} + p_{1e} + p_{1w}$ be the number of pairs of butterflies that share at least a vertex.
%------------------------------------------------
\begin{lem}\label{lem:versamp-var}
$\var{Y} \le \frac{n}{4}(\bfly + p_V)$
\end{lem}
%------------------------------------------------
%------------------------------------------------
\begin{proof}
\erdem{This can be omitted, not sure though}
\erdem{Just keep one proof that uses Fig.3 in the paper. Put the rest in appendix or remove.}
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y} &= \var{\frac{n}{4}\sum_{i=1}^{\bfly}{X_i}} = \frac{n^2}{16} \var{\sum_{i=1}^{\bfly}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov(i, j)} \\
     &= \frac{n^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr}\right] \\
     %&= \frac{n^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr\expec{X_i^2} - \expec{X_i}^2\rbr} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr}\right] \\
     &= \frac{n^2}{16}\left[\bfly \lbr\frac{4}{n} - \frac{16}{n^2}\rbr + \sum_{i\neq{}j}{\lbr\expec{X_iX_j} - \expec{X_i}\expec{X_j}\rbr}\right]
  \end{aligned}
  \end{equation*}
\end{small}
In order to compute $\sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr}$, we examine all kinds of butterfly pairs:
\begin{itemize}
\item
Type $0v$, there is zero probability of $i$ and $j$ being counted within $\bfly_v$, and hence $\expec{X_i X_j} =  0$.
We have $\Cov\lbr X_i, X_j \rbr = -{16}/{n^2}$
\item
Type $1v$, $\E[X_iX_j] = \Pr[X_i=1] \Pr[X_j=1 \vert X_i=1] = ({4}/{n})({1}/{4}) = {1}/{n}$. $\Cov\lbr X_i,X_j \rbr= {1}/{n} - {16}/{n^2}$.
\item
Type $2v$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{n})({1}/{2}) = {2}/{n}$.  $\Cov\lbr X_i,X_j \rbr= {2}/{n} - {16}/{n^2}$.
\item
Type $1e$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{n})({1}/{2}) = {2}/{n}$. $\Cov\lbr X_i,X_j \rbr= {2}/{n} - {16}/{n^2}$.
\item
Type $1w$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{n})({3}/{4}) = {3}/{n}$. $\Cov\lbr X_i,X_j \rbr= {3}/{n} - {16}/{n^2}$.
\end{itemize}
\begin{small}
      \begin{equation*}
      \begin{aligned}
        \Var[Y]  &=  \frac{n^2}{16}\bigg[\bfly \lbr\frac{4}{n} - \frac{16}{n^2}\rbr - p_{0v}\frac{16}{n^2} + p_{1v}(\frac{1}{n}  - \frac{16}{n^2})  \\
                      &  + p_{2v}\lbr\frac{2}{n} - \frac{16}{n^2}\rbr + p_{1e}\lbr\frac{2}{n} - \frac{16}{n^2}\rbr + p_{1w}\lbr\frac{3}{n} - \frac{16}{n^2}\rbr\bigg]\\
         & \leq \frac{n^2}{16}\left[\frac{4}{n}\lbr\bfly + p_{1v} + p_{2v} + p_{1e} + p_{1w}\rbr - {\bfly\choose{2}}\frac{16}{n^2}\right]\\
         & = \frac{n}{4}\lbr\bfly + p_{1v} + p_{2v} + p_{1e} + p_{1w}\rbr - {\bfly\choose{2}} \leq \frac{n}{4}\lbr\bfly + p_V\rbr
      \end{aligned}
      \end{equation*}
\end{small}
\end{proof}
%------------------------------------------------
Let $Z$ be the  average of $\alpha = \frac{8n}{\epsilon^2\bfly}\left(1 + \frac{p_V}{\bfly} \right)$ independent instances of $Y$. We have $\Var[Z] = \Var[Y] / \alpha$.
Using Chebyshev's inequality, we obtain the following:
  \begin{equation*}
  \begin{aligned}
     \prob{|Z - \bfly| \geq \epsilon\bfly}  &\leq \frac{\Var[Z]}{\epsilon^2{}\bfly^2} = \frac{\Var[Y]}{\alpha\epsilon^2{}\bfly^2}
     \leq \frac{n(\bfly + p_V)}{4\alpha\epsilon^2{}\bfly^2} = \frac{1}{32}
  \end{aligned}
  \end{equation*}
We can turn the above estimator that yields an $\epsilon$ relative error with probability $1/32$ into an $(\epsilon,\delta)$ estimator by taking the median of $\bigO(\log(1/\delta))$ estimators, using a standard analysis based on Chernoff bounds (see~\cite{MUbook05}, Chapter 4).
%---------------
\begin{lem}
There is an algorithm that uses $\tilde{\bigO}\left(\frac{n}{\bfly}\left(1 + \frac{p_V}{\bfly} \right) \right)$
iterations~\footnote{We use the notation $\tilde{\bigO}(f)$ to suppress the factor $\frac{\log(1/\delta)}{\epsilon^2}$,
i.e. mean $\bigO\left(f \cdot \frac{\log(1/\delta)}{\epsilon^2}\right)$}
 of \textnormal{\verSam} (\cref{algo:versamp}) and yields an $(\epsilon,\delta)$-estimator of $\bfly(G)$ using expected time $\tilde{\bigO}\left(\frac{m\Delta}{\bfly}\left(1 + \frac{p_V}{\bfly} \right) \right)$. Expected additional space is $\bigO\left(\frac{m\Delta}{n}\right)$.
\end{lem}
%------------
\begin{proof}
An iteration of \textnormal{\verSam} samples a vertex $v$ and calls \textnormal{\pervertex} (\cref{algo:local-verBFC}) for local butterfly counting once, which takes $\bigO(|\Gamma^2_v|)$ time. Hence, the expected runtime of an iteration is $\bigO\left(\expec{|\Gamma^2_v|}\right)$, where the expectation is taken over a uniform random choice of a vertex. We can get a (loose) bound on this expression as follows.  We note that $|\Gamma^2_v| \le d_v~\Delta$ where $d_v$ is $v$'s degree and $\Delta$ is the maximum degree in the graph.
Thus $\expec{|\Gamma^2_v|} \le \sum_{v \in V} \frac{1}{n} d_v \Delta = \frac{\Delta}{n} \sum_{v \in V} d_v = \frac{m\Delta}{n}$.

The space cost of \verSam~{}is same with \textnormal{\pervertex} (\cref{algo:local-verBFC}); $\bigO(|\Gamma_v^2|)$ for handling vertex $v$. The expected value is $\bigO(\frac{m\Delta}{n})$.%Note that the space cost is in addition to the cost of storing the graph itself, which is only needed as read-only access.
\end{proof}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Edge sampling}
We sample a random edge and count the butterflies that this edge participates.
This is done by applying \edgSam~(\cref{algo:local-edgBFC}).~\cref{algo:edgsamp} describes the \edgSam~algorithm. We show that \edgSam~yields an unbiased estimate of $\bfly(G)$.
%-----------------------------------------------------------------------------------------
\begin{algorithm}[t!]
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \Input{A bipartite graph $G = (V, E)$}
    \KwOut{An estimate of $\bfly(G)$}
    Choose an edge $e$ from $E$ uniformly at random.\;
    $\bfly_e \gets \peredge~(e, G)$~\tcp*{\cref{algo:local-edgBFC}}\label{ln:esmp}
%    Compute $\bfly_e$ using \cref{algo:local-edgBFC}\;
    \Return $\bfly_e  \cdot m/4$
    \caption{\edgSam~(single iteration)
    \label{algo:edgsamp}}
\end{algorithm}
%-----------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------
%------------------------------------------------
\begin{lem}
\label{lem:edgsamp-exp}
Let $Y$ denote the return value of \textnormal{\edgSam} (\cref{algo:edgsamp}). Then, $\expec{Y} = \bfly$.
\end{lem}
%------------------------------------------------
%------------------------------------------------
\begin{proof}
\erdem{This can be omitted}
Consider that the butterflies in $G$ are numbered from $1$ to $\bfly$.
Let $X$ denote $\bfly_e$, when edge $e$ is chosen randomly from $E$.
For $i = 1, \ldots, \bfly$, let $X_i$ be an indicator random variable. It is $1$ if edge $e$ is contained in butterfly $i$, and $0$ otherwise.
We have $X = \sum_{i=1}^{\bfly} X_i$. Since each butterfly has exactly four edges in $E$, we have $\prob{X_i=1} = 4/m$.
\begin{align*}
  \expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{m}
\end{align*}
Since $Y = X \cdot \frac{m}{4}$, it follows that $\expec{Y} = \bfly$.
\end{proof}
%------------------------------------------------
Let $p_E$ be the number of pairs of butterflies that share at least one edge. Then, $p_E = p_{1e}+p_{1w}$.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{lem}
$\var{Y} \le \frac{m}{4}(\bfly + p_E)$
\end{lem}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{proof}
Proceeding similar to proof of \cref{lem:versamp-var}:
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y} &= \var{\frac{m}{4}\sum_{i=1}^{\bfly}{X_i}} = \frac{m^2}{16} \var{\sum_{i=1}^{\bfly}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov\lbr i, j\rbr } \\
     &= \frac{m^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr }\right] \\
%     &= \frac{m^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr \expec{X_i^2} - \expec{X_i}^2\rbr } + \sum_{i\neq{}j}{\Cov\lbr i, j\rbr }\right] \\
     &= \frac{m^2}{16}\left[\bfly  \lbr \frac{4}{m} - \frac{16}{m^2}\rbr  + \sum_{i\neq{}j}{\lbr \expec{X_iX_j} - \expec{X_i}\expec{X_j}\rbr }\right]
  \end{aligned}
  \end{equation*}
\end{small}
%  To compute $\sum_{i\neq{}j}{(\expec{X_iX_j} - \expec{X_i}\expec{X_j})}$ we need to consider the different types of pairs of butterflies separately.     %\item
For each type of butterfly pair, we have the following:
\begin{itemize}
\item
Type $0v$, $1v$, or $2v$: there is zero probability of $i$ and $j$ being counted within $\bfly_e$, and hence $\expec{X_i X_j} = 0$. $\Cov \lbr X_i, X_j \rbr = -{16}/{m^2}$
\item
Type $1e$: $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{m})({1}/{4}) = {1}/{m}$. $\Cov\lbr X_i,X_j \rbr= {1}/{m} - {16}/{m^2}$
\item
Type $1w$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{m})({2}/{4}) = {2}/{m}$. $\Cov\lbr X_i,X_j \rbr= {2}/{m} - {16}/{m^2}$
\end{itemize}
\begin{equation*}
  \begin{aligned}
    \Var[Y]  &=  \frac{m^2}{16}\bigg[\bfly \lbr \frac{4}{m} - \frac{16}{m^2}\rbr  - p_{0v}\frac{16}{m^2} - p_{1v}\frac{16}{m^2}  \\
                  &  - p_{2v}\frac{16}{m^2} + p_{1e}\lbr \frac{1}{m} - \frac{16}{m^2}\rbr  + p_{1w}\lbr \frac{2}{m} - \frac{16}{m^2}\rbr \bigg]\\
     & \leq \frac{m^2}{16}\left[\frac{4}{m}\lbr \bfly + p_{1e} + p_{1w}\rbr  - {\bfly\choose{2}}\frac{16}{m^2}\right]\\
     & = \frac{m}{4}\lbr \bfly + p_{1e} + p_{1w}\rbr  - {\bfly\choose{2}} \leq \frac{m}{4}\lbr \bfly + p_E\rbr
  \end{aligned}
\end{equation*}
\end{proof}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
Let $Z$ be the  average of $\alpha = ({8m}\left(1 + {p_E}/{\bfly}\right))/{(\epsilon^2\bfly)}$ independent instances of $Y$.
%We have $\Var[Z] = \Var[Y] / \alpha$.
%= \Var[\frac{1}{\alpha}\sum_{i=1}^{\alpha}Y] = \frac{1}{\alpha^2}\sum_{i=1}^{\alpha}{\Var[Y]} = \frac{\Var[Y]}{\alpha}$.
Using Chebyshev's inequality:
  \begin{equation*}
  \begin{aligned}
     \prob{|Z - \bfly| \geq \epsilon\bfly}  &\leq \frac{\Var[Z]}{\epsilon^2{}\bfly^2} = \frac{\Var[Y]}{\alpha\epsilon^2{}\bfly^2}
     \leq \frac{m(\bfly + p_E)}{4\alpha\epsilon^2{}\bfly^2} = \frac{1}{32}
  \end{aligned}
  \end{equation*}
%We can turn the above estimator that yields an $\epsilon$ relative error with probability $1/32$ into an $(\epsilon,\delta)$ estimator by taking the median of $O(\log(1/\delta))$ estimators, using standard analysis (see for e.g.~{}\cite{MUbook}, Chapter 4).
%---------------
\begin{lem}
There is an algorithm that uses $\tilde{\bigO}\left(\frac{m}{\bfly}\left(1 + \frac{p_E}{\bfly} \right)\right)$ iterations of \textnormal{\edgSam} (\cref{algo:wdgsamp}) and yields an $(\epsilon,\delta)$-estimator of $\bfly(G)$ using time $\tilde{\bigO}\left(\frac{m^2 \Delta}{n\bfly}\left(1 + \frac{p_E}{\bfly} \right)\right)$. The additional space complexity is $\bigO\left(\frac{m\Delta}{n}\right)$.
\end{lem}
%------------
\begin{proof}
\erdem{This can be omitted}
Each iteration of the \edgSam~{}algorithm counts $\bfly_e$ for a randomly chosen $e$. Similar to the analysis of \verSam, the expected time of an iteration is $\bigO(m\Delta/n)$. Hence, the runtime follows. The space complexity is the space taken by \cref{algo:local-edgBFC}, which is $\bigO(m\Delta/n)$.
\end{proof}
%Note that the space cost in the above lemma is in addition to the cost of storing the graph itself, which is only needed as read-only access.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\subsection{Wedge Sampling}
In \wdgSam, we first choose a random ``wedge", which is a path of length two in the graph.
This already yields three vertices that can belong to a potential butterfly.
Then we count the number of butterflies that contain this wedge by finding the intersection of the neighborhoods of the two vertices that are not connected in the wedge.
\cref{algo:wdgsamp} describes the \wdgSam~{}algorithm.

%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{algorithm}[t]
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \Input{A bipartite graph $G = (V, E)$}
    \KwOut{An estimate of $\bfly(G)$}
    $\wdg \gets \sum_{u \in V}{{d_u\choose {2}}}$~\tcp*{number of wedges}
    Choose a vertex $u \in V$ with probability ${{d_u\choose {2}}} / \wdg$\;
    Choose two distinct vertices $v, w \in \Gamma_u$ uniformly at random\;
    $\beta \gets |\Gamma_v \cap \Gamma_w| - 1$~\tcp*{\# butterflies that has $(u, v, w)$}
    \Return $\beta \cdot \wdg/4$\;
    \caption{\wdgSam~(single iteration)}
    \label{algo:wdgsamp}
\end{algorithm}
\begin{lem}
The wedge $(u, v, w)$ in lines 2 and 3 of \cref{algo:wdgsamp} is chosen uniformly at random from the set of all wedges in $G$.
\end{lem}
\begin{proof}
In order to choose the wedge $(u, v, w)$, vertex $u$ must be chosen in step (2), followed by vertices $v$ and $w$ in step (3).
The probability is $({d_y \choose 2}/\wdg) \cdot (1/{d_y \choose 2}) = 1/\wdg$, showing that a wedge is
sampled uniformly at random.
%\red{$\prt{{{d_x\choose {2}}} / \wdg}\prt{1 / {{d_x\choose {2}}}} = 1/\wdg$}. The idea comes from \cite{SePiKo14}.
\end{proof}
%----------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%-----------------------------------------------------------------------------------------------------------------------------------------
\begin{lem}
\label{lem:wdgsamp-exp}
Let $Y$ denote the return value of \cref{algo:wdgsamp}. Then, $\expec{Y} = \bfly$.
\end{lem}
%------------------------------------------------
%------------------------------------------------
\begin{proof}
\erdem{This can be omitted}
Consider that the butterflies in $G = (V, E)$ are numbered from $1$ to $\bfly$.
Suppose that $\wdg$ is the number of wedges in $G$.
For $i = 1, \ldots, \bfly$, let $X_i$ be an indicator random variable equal to $1$ if the $i^{\text{th}}$ butterfly includes wedge $x$.
Let $X$ denote the number of butterflies that contain the sampled wedge $(u, v, w)$.
We have $X = \sum_{i=1}^{\bfly} X_i$. Since each butterfly has four wedges in $G$, we have $\prob{X_i=1} = 4/\wdg$. The rest of the proof
 is similar to that of \cref{lem:versamp-exp}, and is omitted.
%  \begin{equation*}
%  \begin{aligned}
%        \expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{\wdg}
%  \end{aligned}
%  \end{equation*}
%Since $Y = X \times \frac{\wdg}{4}$, it follows that $\expec{Y} = \bfly$.
\end{proof}

%Let $p_w$ denote the number of pairs of butterflies that share a wedge.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{lem}
$\var{Y} \le \frac{\wdg}{4}(\bfly + p_{1w})$
\end{lem}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{proof}
\erdem{This can be omitted}
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y} &= \var{\frac{\wdg}{4}\sum_{i=1}^{\bfly}{X_i}} = \frac{\wdg^2}{16} \var{\sum_{i=1}^{\bfly}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov\lbr i, j\rbr } \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr }\right] \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr \expec{X_i^2} - \expec{X_i}^2\rbr } + \sum_{i\neq{}j}{\Cov\lbr i, j\rbr }\right] \\
     &= \frac{\wdg^2}{16}\left[\bfly \lbr \frac{4}{\wdg} - \frac{16}{\wdg^2}\rbr  + \sum_{i\neq{}j}{\lbr \expec{X_iX_j} - \expec{X_i}\expec{X_j}\rbr }\right]
  \end{aligned}
  \end{equation*}
\end{small}
 % To compute $\sum_{i\neq{}j}{(\expec{X_iX_j} - \expec{X_i}\expec{X_j})}$: {\iffalse we need to consider the different types of pairs of butterflies separately. \fi}    %\item
 For a butterfly pair $(i,j)$, we have the following options;
\begin{itemize}
\item
Type $0v$, $1v$, $2v$, or $1e$, there is zero probability of $i$ and $j$ being counted together, and hence $\expec{X_i X_j}  = 0$. We have $\Cov \lbr X_i, X_j \rbr = -{16}/{\wdg^2}$
\item
Type $1w$, $\E[X_iX_j] = \Pr[X_i=1]\Pr[X_j=1|X_i=1] = ({4}/{\wdg})({1}/{4}) = {1}/{\wdg}$. Therefore, $\Cov\lbr X_i,X_j \rbr= {1}/{\wdg} - {16}/{\wdg^2}$.
\end{itemize}
\begin{equation*}
  \begin{aligned}
    \Var[Y]  &=  \frac{\wdg^2}{16}\bigg[\bfly \lbr \frac{4}{\wdg} - \frac{16}{\wdg^2}\rbr  - p_{0v}\frac{16}{\wdg^2} - p_{1v}\frac{16}{\wdg^2}  \\
                  &  - p_{2v}\frac{16}{\wdg^2} - p_{1e}\frac{16}{\wdg^2} + p_{1w}\lbr \frac{1}{\wdg} - \frac{16}{\wdg^2}\rbr \bigg]\\
     & \leq \frac{\wdg^2}{16}\left[\frac{4}{\wdg}\lbr \bfly + p_{1w}\rbr  - {\bfly\choose{2}}\frac{16}{\wdg^2}\right]\\
     & = \frac{\wdg}{4}\lbr \bfly + p_{1w}\rbr  - {\bfly\choose{2}} \leq \frac{\wdg}{4}\lbr \bfly + p_{1w}\rbr
  \end{aligned}
\end{equation*}
\end{proof}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
Let $Z$ be the  average of $\alpha = ({8\wdg}\left(1 + {p_{1w}}/{\bfly}\right))/{(\epsilon^2\bfly)}$ independent instances of $Y$.
Using Chebyshev's inequality, we arrive that $Z$ is an $(\epsilon, 1/32)$-estimator of $\bfly(G)$.
%We have $\Var[Z] = \Var[Y] / \alpha$.
%= \Var[\frac{1}{\alpha}\sum_{i=1}^{\alpha}Y] = \frac{1}{\alpha^2}\sum_{i=1}^{\alpha}{\Var[Y]} = \frac{\Var[Y]}{\alpha}$.
%Using Chebyshev's inequality, we have:
%  \begin{equation*}
%  \begin{aligned}
%     \prob{|Z - \bfly| \geq \epsilon\bfly}  &\leq \frac{\Var[Z]}{\epsilon^2{}\bfly^2} = \frac{\Var[Y]}{\alpha\epsilon^2{}\bfly^2}
%    \leq \frac{\wdg(\bfly + p_{1w})}{4\alpha\epsilon^2{}\bfly^2} = \frac{1}{32}
%  \end{aligned}
%  \end{equation*}

%We can turn the above estimator that yields an $\epsilon$ relative error with probability $1/32$ into an $(\epsilon,\delta)$ estimator by taking the median of $O(\log(1/\delta))$ estimators, using standard analysis (see for e.g.~{}\cite{MUbook}, Chapter 4).
%---------------
\begin{lem}
There is an algorithm that uses $\allowbreak\tilde{\bigO}\bigl(\frac{\wdg}{\bfly}\bigl(1 + \frac{p_{1w}}{\bfly} \bigr)\bigr)$
iterations of \cref{algo:wdgsamp} and yields an $(\epsilon,\delta)$-estimator of $\bfly(G)$ using time $\tilde{\bigO}\left(\frac{(\Delta + \log n)\wdg}{\bfly}\left(1 + \frac{p_{1w}}{\bfly} \right)\right)$ and space $\bigO(n)$.
\end{lem}
%------------
\begin{proof}
\erdem{This can be omitted}
We first consider the runtime of \cref{algo:wdgsamp}. At first glance, it looks like Steps (1) and (2) take $\bigO(n)$ time.
This can be reduced to $\bigO(\log n)$ using a pre-computation step of time $\bigO(n)$, which precomputes the value of $h$, and also stores
the values of ${d_v \choose 2}$ for different vertices $v$ in an array $A[1\ldots n]$ of length $n$. We consider another array $B[1\ldots n]$, where each element $B[j] = \sum_{i=1}^j A[i]$.  When \wdgSam~{}is called, a random number $r$ in the range $\{1,2,\ldots,h\}$ is first generated, and Step (2) is accomplished through finding the smallest $j$ such that $B[j] \ge r$. Since array $B$ is sorted in increasing order, this can be done in time $\bigO(\log n)$ using a binary search. Steps (3) and (4) of \cref{algo:wdgsamp} can be performed in $\bigO(\Delta)$ time -- Step (4), for example, through storing all elements of $\Gamma_u$ in a hash set, and repeatedly querying for elements of $\Gamma_v$ in this hash set, for a total of $\bigO(d_v) = \bigO(\Delta)$ time. The additional space required by this algorithm, in addition to the stored graph itself, is $\bigO(n)$, for random sampling.
\end{proof}
%Note that the space cost in the above lemma is in addition to the cost of storing the graph itself, which is only needed as read-only access.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%\subsection{Comparison}
%We next compare the different sampling algorithms




\subsection{Comparison of variances on real-world networks}

In order to understand the relation between these three, we compare the variance of the estimates retuned by these algorithms. Note that each of them returns an unbiased estimate of the number of butterflies.
The variance of \verSam, \edgSam, and \wdgSam~{}for different graphs are estimated and summarized in \cref{table:variance-sam}. The results show that the variances of \verSam~{}and \wdgSam~{}are much higher than the variance of \edgSam. 

%
%%-------------- old table
%\begin{table}[b!]
%	\vspace{1ex}
%	\centering
%	\resizebox{0.5\textwidth}{!}{
%		\begin{tabular}{|c| @{\extracolsep{\fill}} |c|c|c|}
%			\hline
%	\multirowcell{2.3}[1.9ex]{\diagbox[height=1.95\line]{\rlap{\enspace\raisebox{0.6ex}{Graph}}}{\raisebox{-0.5ex}{Algorithm}}} & \makecell{\verSam{}\\$(\bfly + p_v)n/4$} & \makecell{\edgSam\\$(\bfly + p_e)m/4$} & \makecell{\wdgSam\\$(\bfly + p_w)h/4$} \\\hline
%	
%			\deli & $7.928 \times 10^{26}$ & $1.628 \times 10^{18}$ & $6.033 \times 10^{23}$ \\ \hline		
%			\jrn & $5.458 \times 10^{30}$ & $5.584 \times 10^{24}$ & $2.046 \times 10^{28}$\\ \hline
%			\ork & $2.450 \times 10^{31}$ & $5.290 \times 10^{21}$ & $1.031 \times 10^{29}$ \\ \hline
%			\web & $4.742 \times 10^{33}$ & $1.073 \times 10^{22}$ & $1.940 \times 10^{33}$ \\ \hline
%			\wiki & $1.931 \times 10^{32}$ & $6.818 \times 10^{19}$ & $2.052 \times 10^{30}$\\ \hline
%	\end{tabular}}
%	\vspace{1ex}
%	\caption{Variance values for the sampling estimators given in \cref{sec:sampling} on the large graphs}\label{table:variance-sam}
%\end{table}
%%--------------



\begin{table}[t!]
\footnotesize
%\hspace{-7ex}
\centering
\begin{tabular}{|c|c|r|c|r|c|r|c|}\hline
& \multicolumn{2}{c|}{\verSam} & \multicolumn{2}{c|}{\edgSam} & \multicolumn{2}{c|}{\wdgSam} \\
& $\frac{(\bfly+p_V)n}{4}$ & error \% & $\frac{(\bfly+p_E)m}{4}$ & error \% & $\frac{(\bfly+p_{1w})h}{4}$ & error \% \\ \hline
\deli	&	$	7.9\times 10^{26}	$	&	$	495	$	&	$  4.7 \times 10^{24}	$	&	$	xxx	$	&	$	6.0\times 10^{23}	$	&	$	14	$	\\ \hline
\jrn	&	$	5.5\times 10^{30}	$	&	$	709	$	&	$  4.5 \times 10^{26}	$	&	$	xxx	$	&	$	2.0\times 10^{28}	$	&	$	43	$	\\ \hline
\ork	&	$	2.5\times 10^{31}	$	&	$	224	$	&	$	4.1 \times 10^{28}	$	&	$  xxx	$	&	$	1.0\times 10^{29}	$	&	$	15	$	\\ \hline
\web	&	$	4.7\times 10^{33}	$	&	$	3432	$	&	$ 1.6 \times 10^{34}	$	&	$	xxx	$	&	$	1.9\times 10^{33}	$	&	$	2195	$	\\ \hline
\wiki	&	$	1.9\times 10^{32}	$	&	$	6824	$	&	$ 1.5 \times 10^{27}	$	&	$	xxx	$	&	$	2.1\times 10^{30}	$	&	$	703	$	\\ \hline
	\end{tabular}
	\vspace{1ex}
	\caption{Variance values for the sampling estimators given in \cref{sec:sampling} on the large graphs. \erdem{Errors are sqrt of variance numbers over the num of butterflies. For vertex and wedge those upper bound are correct. but i didn't understand it for edge sampling? We do have errors more than those numbers (in figs 5-8). any idea?}}\label{table:variance-sam}
\end{table}


%Let us compare the variances of \verSam~{}and \edgSam.  
The variance of \verSam~{}is proportional to $n p_V$ where $p_V$ is the number of {\em pairs of butterflies that share a vertex} and $n$ is the number of vertices. 
For the \edgSam, the variance is correlated with $m p_E$ where $p_E$ is the number of {\em pairs of butterflies that share an edge} and $m$ is the number of edges
Note that typically $\bfly \ll p_V, p_E$ and hence $\bfly + p_V \approx p_V$ and $\bfly + p_E \approx p_E$.
If two butterflies share an edge, they certainly share a vertex, hence $p_E \le p_V$. Since it is possible that two butterflies share a vertex but do not share an edge, $p_E$ could be much smaller than $p_V$.
It turns out that in most of these graphs, $p_E$ was much smaller than $p_V$.
On the other hand, the number of vertices in a graph ($n$) is comparable to the number of edges ($m$). Typically $m < 10n$, and only in one case (\ork), we have $m \approx 30n$.
Thus, $n p_V \ll m p_E$ for the graphs we consider. 
As a result, the variance of \verSam~{}estimator is much larger than the variance of \edgSam{}, which is reflected clearly in \cref{table:variance-sam}. 
%This explains why \verSam~{}performs poorly when compared with \edgSam. 

Regarding the comparison of \edgSam~{}with \wdgSam, we note that the variance of \wdgSam~{}is proportional to $\wdg p_{1w}$, where $\wdg$ is the number of wedges in the graph, which is $\bigO(\sum_v d_v^2)$ and $p_{1w}$ is the number of pairs of butterflies that share a wedge.
The variance for \edgSam is correlated with $m p_E$, as mentioned above. 
$p_1w \le p_E$ since each pair of butterflies that shares a wedge also shares an edge.
At the same time, we see that $\wdg$ is substantially greater than $m$. 
Overall, the variance of \wdgSam~{}is larger than that of \edgSam, and \edgSam~{}has the smallest variance among all.
%Due to high variance on large graphs, \verSam and \wdgSam~{}do not converge to less than one percent error. In the graph \deli, the variance of \wdgSam~{}is not too much. \cref{figure:deli-sam-err-time} shows that this algorithm estimates the number of butterflies within one percent error after a few seconds.

\subsection{Runtime discussion}\label{sec:quickBFC}

Here we study the time taken by the different sampling algorithms. \cref{figure:timePerSample} presents the results for the largest five networks in our dataset.
Note that, sampling the same number vertices/edge/wedges shows that \edgSam~gives much less variance than the others.
However, \edgSam~{}requires the largest amount of time per sampling step with a significant difference. This decreases the overall efficiency of the \edgSam~{}algorithm despite its small variance observed in~\cref{table:variance-sam}. 

\begin{figure}[!t]
\centering
\resizebox{0.7\linewidth}{!}{\input{newResults/histogram/time-per-sample}}
\caption{{\small Avg. time to get one sample for sampling algorithms.}\erdem{make it smaller and also remove the fast edge sampling bars (will be shown in~\cref{sec:quickBFC})}}
\label{figure:timePerSample}
\vspace{-1ex}
\end{figure}


\subsubsection{Speeding up the edge sampling:~\textnormal{\fstEdg}}
In order to reduce the time taken by each iteration of~\edgSam, we propose another level of sampling,~\fstEdg, that estimates the number of butterflies for a given edge.
Instead of computing the exact number of butterflies for each edge $(u, v)$ (line~\ref{ln:esmp} of \edgSam~(\cref{algo:edgsamp})), we randomly choose one neighbor of $u$ and of $v$, and check if those four vertices form a butterfly.
\cref{algo:qBFC} presents the~\fstEdg algorithm.
We use it instead of the \peredge algorithm in \edgSam.
We expect that while the estimate from each iteration is less accurate than in \edgSam, each iteration is faster, so that more iterations are possible within the same time.
Overall, in large graphs, this leads to an improvement in accuracy over \edgSam. For a given edge $e$, \cref{algo:qBFC} yields an unbiased estimate of $\bfly_e$.

\begin{algorithm}[t!]
    \DontPrintSemicolon
    \KwIn{An edge $e = (v, u) \in E$ in $G = (V, E)$}
    \KwOut{An estimate of $\bfly_e$}
    Choose a vertex $w$ ($\ne v$) from $\Gamma_u$ uniformly at random\;
    Choose a vertex $x$ ($\ne u$) from $\Gamma_v$ uniformly at random\;
    \IfThen{$(u, v, w, x)$ forms a butterfly}{${\beta} \gets 1$}\;
    \lElse {${\beta} \gets 0$}
    \Return ${\beta}\cdot (d_u-1) \cdot (d_v-1)$\;
    \caption{\fstEdg~(replaces \peredge~in \edgSam)
    \label{algo:qBFC}}
\end{algorithm}

\begin{lem}
\label{lem:fastedge-samp-exp}
Let $Y$ denote the return value of \cref{algo:qBFC}. Then, $\expec{Y} = \bfly_e$
\end{lem}
%------------------------------------------------
%------------------------------------------------
\begin{proof}
Consider that the butterflies include the edge $e = (u, v)$ are numbered from $1$ to $\bfly_e$.
For $i = 1, \ldots, \bfly_e$, let $X_i$ be an indicator random variable. $X_i$ is equal $1$ if the $i^{\text{th}}$ butterfly contains both sampled neighbors $w$ and $x$, otherwise $0$.
Let $X = \sum_{i=1}^{\bfly_e} X_i$. Since vertex $w$ and $x$ are chosen with probability $1/d_u$ and $1/d_v$, respectively, $\prob{X_i=1} = 1/(d_u \cdot d_v)$. Then,
\begin{align*}
  \expec{X} = \sum_{i=1}^{\bfly_e} \expec{X_i} = \sum_{i=1}^{\bfly_e} \prob{X_i=1} = \frac{\bfly_e}{d_u\cdot{}d_v}
\end{align*}
$Y = X \cdot d_u \cdot d_v$ follows that $\expec{Y} = \bfly_e$.
%  \begin{equation*}
%  \begin{aligned}
%        \expec{X} = \sum_{i=1}^{\bfly} \expec{X_i} = \sum_{i=1}^{\bfly} \prob{X_i=1} = \frac{4\bfly}{\wdg}
%  \end{aligned}
%  \end{equation*}
%Since $Y = X \times \frac{\wdg}{4}$, it follows that $\expec{Y} = \bfly$.
\end{proof}
%Let $p_w$ denote the number of pairs of butterflies that share a wedge.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{lem}
$\var{Y} \leq \bfly_e(d_u \cdot d_v)$
\end{lem}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\begin{proof}
\begin{small}
  \begin{equation*}
  \begin{aligned}
    \var{Y} &= \var{(d_u \cdot d_v)\sum_{i=1}^{\bfly_e}{X_i}} = (d_u \cdot d_v)^2~{}\var{\sum_{i=1}^{\bfly_e}{X_i}} \\ %\frac{n^2}{4}\sum_{i=1}^{\bfly}\sum_{j=1}^{\bfly}{\Cov\lbr i, j\rbr } \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i=1}^{\bfly}{\var{X_i}} + \sum_{i\neq{}j}{\Cov\lbr X_i, X_j\rbr }\right] \\
%     &= \frac{\wdg^2}{16}\left[\sum_{i = 1}^{\bfly}{\lbr \expec{X_i^2} - \expec{X_i}^2\rbr } + \sum_{i\neq{}j}{\Cov\lbr i, j\rbr }\right] \\
%     &= (d_v \cdot d_u)^2\left[\sum_{i=1}^{\bfly_e}{\left[\expec{X_i^2} - \expec{X_i}^2\right]} + \sum_{i \neq j}{\Cov(X_i, X_j)}\right]\\
     &= (d_u \cdot d_v)^2\left[\sum_{i=1}^{\bfly_e}{\left[\frac{1}{d_u \cdot d_v} - \frac{1}{(d_u \cdot d_v)^2}\right]} - {\bfly_e \choose {2}}\right]\\
     &\le \bfly_e \cdot d_u \cdot d_v
  \end{aligned}
  \end{equation*}
\end{small}
 % To compute $\sum_{i\neq{}j}{(\expec{X_iX_j} - \expec{X_i}\expec{X_j})}$: {\iffalse we need to consider the different types of pairs of butterflies separately. \fi}    %\item
\end{proof}
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
Let $Z$ be the  average of $\alpha = 32({d_u\cdot{}d_v})/{(\epsilon^2\bfly_e)}$ independent instances of $Y$.
Using Chebyshev's inequality, we arrive that $Z$ is an $(\epsilon, 1/32)$-estimator of $\bfly_e$.
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\subsubsection{\textnormal{\fstEdg}~runtime}



\begin{table}[t!]
\footnotesize
%\hspace{-7ex}
\centering
\begin{tabular}{|c|r|r|r|}\hline
%& \multicolumn{2}{c|}{\verSam} & \multicolumn{2}{c|}{\edgSam} & \multicolumn{2}{c|}{\wdgSam} \\
%& $\frac{(\bfly+p_V)n}{4}$ & error \% & $\frac{(\bfly+p_E)m}{4}$ & error \% & $\frac{(\bfly+p_{1w})h}{4}$ & error \% \\ \hline
in & \multicolumn{2}{c|}{\edgSam} &   \\
milliseconds & with \peredge & with \fstEdg  & Speedup \\ \hline
\deli	&	$	2.61	$	&	$	0.17	$	&	$	15.4	$	\\ \hline
\jrn	&	$	172.42	$	&	$	0.48	$	&	$	357.4	$	\\ \hline
\ork	&	$	36.76	$	&	$	0.37	$	&	$	98.1	$	\\ \hline
\web	&	$	34.49	$	&	$	0.42	$	&	$	81.5	$	\\ \hline
\wiki	&	$	55.65	$	&	$	0.48	$	&	$	115.5	$	\\ \hline
\end{tabular}
\vspace{1ex}
\caption{Runtimes of \edgSam~algorithms per iteration when \peredge~and \fstEdg~are used. Speedup of the second over first is given in the last column}\label{tab:quickBFC}
\end{table}

\cref{tab:quickBFC} gives the comparison of \peredge~and \fstEdg~when they are used in the \edgSam.
We observe speedups from $15.4$ up to $357.4$ per each iteration.

\subsection{Comparing all sampling approaches}

We compare all the sampling algorithms: \verSam~(\cref{algo:versamp}), \edgSam~(\cref{algo:edgsamp}) with \peredge, \edgSam with~\fstEdg~(\cref{algo:qBFC}), and \wdgSam~(\cref{algo:wdgsamp}) in terms of their accuracy and efficiency. We show the results for the five large bipartite graphs. A sampling algorithm immediately starts producing estimates that typically get better as more iterations of sampling take place. We record the number of iterations and relative percent error of sampling algorithms up to 60 seconds. \cref{figure:deli-sam-err-time,figure:jrn-sam-err-time,figure:ork-sam-err-time,figure:web-sam-err-time,figure:wiki-sam-err-time} show the relative percent error with respect to the runtime.



%\begin{figure}[!t]
%\centering
%\captionsetup[subfigure]{captionskip=-3ex}
%\subfloat[\footnotesize \deli]{\input[width=0.19\linewidth]{newResults/delicious/sam-err-time}}
%\subfloat[\footnotesize \ork]{\input[width=0.19\linewidth]{newResults/orkut/sam-err-time}}
%\subfloat[\footnotesize \jrn]{\input[width=0.19\linewidth]{newResults/Journal/sam-err-time}}
%\subfloat[\footnotesize \web]{\input[width=0.19\linewidth]{newResults/trackers/sam-err-time}}
%\subfloat[\footnotesize \wiki]{\input[width=0.19\linewidth]{newResults/Wikipedia/sam-err-time}}
%\hspace{-5ex}
%\subfloat[\footnotesize \textbf{\textsc{$(2,3)$ nucleus}}]{\includegraphics[width=0.6\linewidth]{./figures/mov_23_new.pdf}}
%\hspace{-13ex}
%
%\hspace{-1ex}
%\vspace{-7.5ex}
%\caption{\footnotesize \bf Dense subgraphs for the \imdb~network. Each dot is a bipartite subgraph and edge density is color coded. $U'$ and $V'$ are the primary and secondary vertex sets and their sizes are given on the x- and y-axes. Wing decomposition results in 36 bipartite subgraphs with $\ge 0.9$ edge density that have at least 10 vertices in each side, and perform competitive to the butterfly densest subgraph~\protect{\cite{Babis15KDD}}. Other algorithms working on projections, on the right, cannot report any bipartite subgraphs in that quality.}
%\vspace{0ex}
%\label{fig:introfig}
%\end{figure}



\begin{figure*}[!t]
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/delicious/sam-err-time}}
		\caption {\deli}\label{figure:deli-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/Journal/sam-err-time}}
		\caption {\jrn}\label{figure:jrn-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/orkut/sam-err-time}}
		\caption {\ork}\label{figure:ork-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/trackers/sam-err-time}}
		\caption {\web}\label{figure:web-sam-err-time}
	\end{minipage}
	\begin{minipage}{.19\linewidth}
		\centering
		\resizebox{\linewidth}{!}{\input{newResults/Wikipedia/sam-err-time}}
		\caption {\wiki.}\label{figure:wiki-sam-err-time}
	\end{minipage}
	\vspace{1ex}
	\caption*{{\bf Accuracy by time results for sampling algorithms.}~\fstEdg~{\bf results in less than one percent relative error within 7 seconds for all the networks.}\erdem{replace those with the new 30 trial results and edit the text as needed. And please put pdfs of the figures. we can remove one of five for brevity. Also, put those in a proper subfigure format}}
	\vspace{-1ex}
\end{figure*}

The experiments on sampling show that \verSam~{}performs poorly when compared with \edgSam~{}and \wdgSam under the same time budget. The performance of \edgSam~{}is typically (but not always) better than that of \wdgSam.
As we show in~\cref{table:variance-sam}, \edgSam~gives way better variance results than \wdgSam. However, since \wdgSam~is faster than~\edgSam per iteration, more iterations of \wdgSam~are possible given the same time budget.
For instance, applying 1000 iterations in \wiki~network results in $51\%$ error with \wdgSam~whereas the \edgSam~can yield $29\%$ error. But, the former takes $0.13$ seconds while the latter needs $33.76$ secs.
Considering all the graphs, using \fstEdg~yields the best results; \textbf{less than one percent relative error can be reported within $7$ seconds}.
%\erdem{any explanation for that? Deli, orkut, and wiki are like that. Oh ok. This is because we show the time in x-axis. We KNOW that if the same number of samples are used, edge sampling definitely outperforms wedge sampling -- I also checked the raw data. But we need to state this explicitly.}









==> setup.tex <==
%----------------------------------------
\section{Networks and Experimental Setup}
%----------------------------------------
We used massive real-world bipartite networks, selected from the publicly available KONECT network repository 
\footnote{\url{http://konect.uni-koblenz.de/}}. The graphs that we have used are summarized in~{}\cref{table:graphs}. 
We converted all graphs to simple, undirected graphs by removing edge directions (if graph was directed),  and by removing all self-loops, multiple edges, and isolated vertices (vertices with degree zero).
We implemented all algorithms in C++,  compiled with Visual C++ 2015 compiler (Version 14.0), and report the runtimes on a machine equipped with a $3.50$ GHz Intel(R) Xeon(R) CPU E3-1241 v3 and a $16.0$ GB memory. 


\begin{table}[t!]
\footnotesize
	\centering
	\renewcommand{\tabcolsep}{1pt}
%	\resizebox{0.5\textwidth}{!}{
		\begin{tabular}{|c| @{\extracolsep{\fill}} |r|r|r|r|r|r|}
			\hline
			Bipartite graph     & $|L|$  & $|R|$ & $|E|$ & $\sum_{\ell\in{}L}{d_\ell^2}$ & $\sum_{r\in{}R}{d_r^2}$ & $\bfly$ \\ \hline
			\texttt{$\prt{10^4,10}$-biclique} & \num{10}K & \num{10} & \num{100}K & \num{1}M & \num{1}B & \num{2.2}B \\ \hline
			\href{http://konect.uni-koblenz.de/networks/dbpedia-location}{\texttt{DBPedia-Location}}    & \num{172}K & \num{53}K & \num{293}K & \num{629}K & \num{245}M & \num{3.7}M \\ \hline
			\href{http://konect.uni-koblenz.de/networks/edit-frwiki}{\wikiFR}    & \num{288}K & \num{3.9}M & \num{22}M & \num{2.1}T & \num{795}M & \num{601}B \\ \hline
			\href{http://konect.uni-koblenz.de/networks/munmun_twitterex_ut}{\twt}   & \num{175}K & \num{530}K & \num{1.8}M & \num{74.1}M & \num{1.9}B & \num{206}M \\ \hline
			\href{http://konect.uni-koblenz.de/networks/amazon-ratings}{\amz}    & \num{2.1}M & \num{1.2}M & \num{5.7}M & \num{828}M & \num{437}M & \num{35.8}M  \\ \hline
			\href{http://konect.uni-koblenz.de/networks/livejournal-groupmemberships}{\jrn}     & \num{3.2}M & \num{7.4}M & \num{112}M & \num{9.5}B & \num{5.4}T & \num{3.3}T  \\ \hline
			\href{http://konect.uni-koblenz.de/networks/edit-enwiki}{\wiki}     & \num{3.8}M & \num{21.4}M & \num{122}M & \num{12.5}T & \num{23.2}B & \num{2}T  \\ \hline
			\href{http://konect.uni-koblenz.de/networks/delicious-ui}{\deli}     & \num{833}K & \num{33.7}M & \num{101}M & \num{85.9}B & \num{52.7}B & \num{56.8}B  \\ \hline
			\href{http://konect.uni-koblenz.de/networks/orkut-groupmemberships}{\ork}    & \num{2.7}M & \num{8.7}M & \num{327}M & \num{156}M & \num{4.9}T & \num{22.1}T  \\ \hline
			\href{http://konect.uni-koblenz.de/networks/trackers-trackers}{\web}  & \num{27.6}M & \num{12.7}M & \num{140}M & \num{1.7}B & \num{211}T  & \num{20}T   \\ \hline
		\end{tabular}
%	}
%	\vspace*{-0cm}
	\caption{\small Bipartite network datasets. $L$ and $R$ are the partitions of the vertex set, $E$ is the set of edges, and next two columns are the sum of the degree squares for $L$ and $R$, respectively. Number of butterflies is given in the last column.
	\label{table:graphs}}
	\vspace{-8ex}
\end{table}

%\begin{table*}[t!]
%\scriptsize
%	\centering
%	\resizebox{0.75\textwidth}{!}{
%		\begin{tabular}{|c| @{\extracolsep{\fill}} |r|r|r|r|r|r|}
%			\hline
%			Bipartite graph     & $|L|$  & $|R|$ & $|E|$ & $\sum_{\ell\in{}L}{d_\ell^2}$ & $\sum_{r\in{}R}{d_r^2}$ & $\bfly$ \\ \hline
%			\texttt{$\prt{10^4,10}$-biclique} & \num{10000} & \num{10} & \num{100000} & \num{1000000} & \num{1000000000} & \num{2249775000} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/dbpedia-location}{\texttt{DBPedia-Location}}    & \num{172079} & \num{53407} & \num{293697} & \num{629983} & \num{245744643} & \num{3761594} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/edit-frwiki}{\wikiFR}    & \num{288275} & \num{3992426} & \num{22090703} & \num{2186560482259} & \num{795544489} & \num{601291038864} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/munmun_twitterex_ut}{\twt}   & \num{175214} & \num{530418} & \num{1890661} & \num{74184693} & \num{1943171143} & \num{206508691} \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/amazon-ratings}{\amz}    & \num{2146057} & \num{1230915} & \num{5743258} & \num{828704126} & \num{437163474} & \num{35849304}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/livejournal-groupmemberships}{\jrn}     & \num{3201203} & \num{7489073} & \num{112307385} & \num{9565595799} & \num{5398290985343} & \num{3297158439527}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/edit-enwiki}{\wiki}     & \num{3819691} & \num{21416395} & \num{122075170} & \num{12576726351444} & \num{23256846234} & \num{2036443879822}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/delicious-ui}{\deli}     & \num{833081} & \num{33778221} & \num{101798957} & \num{85945241607} & \num{52787267117} & \num{56892252403}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/orkut-groupmemberships}{\ork}    & \num{2783196} & \num{8730857} & \num{327037487} & \num{156580049011} & \num{4900153043329} & \num{22131701213295}  \\ \hline
%			\href{http://konect.uni-koblenz.de/networks/trackers-trackers}{\web}  & \num{27665730} & \num{12756244} & \num{140613762} & \num{1733678094524} & \num{211149951033914}  & \num{20067567209850}   \\ \hline
%		\end{tabular}
%	}
%%	\vspace*{-0cm}
%	\caption{Bipartite network datasets. $L$ and $R$ are the partitions of the vertex set, $E$ is the set of edges, and next two columns are the sum of the degree squares for $L$ and $R$, respectively. Number of butterflies is given in the last column.
%	\label{table:graphs}}
%\end{table*}

%We present the results of an experimental evaluation of our algorithms for butterfly counting. We implemented the different algorithms \exact, \clr, \edgSpr, \verSam, \wdgSam, \edgSam, and \fstEdg. Based on their approach, they are classified as: (1)~{}Exact Algorithm (\exact)~{}which computes the exact number of butterflies in a bipartite graph (2)~{}Sparsification-based algorithms, \clr~{}and \edgSpr, and (3)~{}Sampling algorithms, \verSam, \wdgSam, \edgSam, and \fstEdg. For comparison, we also implemented the algorithm of Wang, Fu, and Cheng~{}\cite{Wang14}, which we call as \wangExact.
%We report the following statistics: (1)~{}Relative percent error of the estimate, equal to $100 \times (|\bfly - Y|) / \bfly $ where $\bfly$ is the exact number of butterflies in $G$, and $Y$ is the estimate returned by the algorithm. (2)~{}The time taken by the algorithm. For each data point, we report the median of the fifteen trials.


%\begin{table}[t!]
%\scriptsize
%%\hspace{-7ex}
%\centering
%\begin{tabular}{|c|c|r|c|r|c|r|c|}\hline
%& \multicolumn{2}{c|}{\verSam} & \multicolumn{2}{c|}{\edgSam} & \multicolumn{2}{c|}{\wdgSam} \\
%& $(\bfly+p_V)n/4$ & error \% & $(\bfly+p_E)m/4$ & error \% & $(\bfly+p_{1w})h/4$ & error \% \\ \hline
%\deli	&	$	7.9\times 10^{26}	$	&	$	495	$	&	$	1.6\times 10^{18}	$	&	$	0.022	$	&	$	6.0\times 10^{23}	$	&	$	14	$	\\ \hline
%\jrn	&	$	5.5\times 10^{30}	$	&	$	709	$	&	$	5.6\times 10^{24}	$	&	$	0.717	$	&	$	2.0\times 10^{28}	$	&	$	43	$	\\ \hline
%\ork	&	$	2.5\times 10^{31}	$	&	$	224	$	&	$	5.3\times 10^{21}	$	&	$	0.003	$	&	$	1.0\times 10^{29}	$	&	$	15	$	\\ \hline
%\web	&	$	4.7\times 10^{33}	$	&	$	3432	$	&	$	1.1\times 10^{22}	$	&	$	0.005	$	&	$	1.9\times 10^{33}	$	&	$	2195	$	\\ \hline
%\wiki	&	$	1.9\times 10^{32}	$	&	$	6824	$	&	$	6.8\times 10^{19}	$	&	$	0.004	$	&	$	2.1\times 10^{30}	$	&	$	703	$	\\ \hline
%	\end{tabular}
%	\vspace{1ex}
%	\caption{Variance values for the sampling estimators given in \cref{sec:sampling} on the large graphs}\label{table:variance-sam}
%\end{table}


